FARSI: Facebook AR System Investigator for Agile Domain-Specific System-on-Chip Exploration

Domain-specific SoCs (DSSoCs) are attractive solutions for domains with stringent power/performance/area constraints; however, they suffer from two fundamental complexities. On the one hand, their many specialized hardware blocks result in complex systems and thus high development effort. On the other, their many system knobs expand the complexity of design space, making the search for the optimal design difficult. Thus to reach prevalence, taming such complexities is necessary. This work identifies necessary features of an early-stage design space exploration (DSE) framework that targets the complex design space of DSSoCs and further provides an instance of one called FARSI, (F)acebook (AR) (S)ystem (I)nvestigator. Concretely, FARSI provides an agile system-level simulator with speed up and accuracy of 8,400X and 98.5% comparing to Synopsys Platform Architect. FARSI also provides an efficient exploration heuristic and achieves up to 16X improvementin convergence time comparing to naive simulated annealing (SA). This is done by augmenting SA with architectural reasoning such as locality exploitation and bottleneck relaxation. Furthermore, we embed various co-design capabilities and show that on average, they have a 32% impact on the convergence rate. Finally, we demonstrate that using simple development-cost-aware policies can lower the system complexity, both in terms of the component count and variation by as much as 150% and 118% (e,g., for Network-on-a-Chip subsystem)

==> tex/AGDSE.tex <==
previous work \red{cite a bunhc of work}, characterizes the space with parameters/knobs. Then proceeds to use various architectural-obiivious search aglrithms to find the optimal design. In contrast, our work uses transformations and schedules them to improvethe design. 

==> tex/dep/ECC.tex <==
\section{flow} \label{sec:ECC} 
Dynamic world, Static design


How does dynamicity manifest itself

consider the velocity/response time interaction. 
space/resolution interaction. space response time.

what are the knobs:
reactive knobs. These are the knobs where the impact is contained to the compute, i.e., the runtime controls the compute.
        map resolution
        map volume communicated
        number of iterations in the planner
    

proactive knobs. These are the knobs that go beyond compute, i.e, compute pushes back on the sensors and actuators.
    FOV 
    possibly range 
    max velocity (controlls slack in space)



there are two main questions to be ask now?
how does the run time decides on the parameter values? (run time policy. We advocate a space/time based slack policy).
slack in space for sensors and slack in time for actuators.
How does FOV and max velocity come into play?



all the knobs seem to target volume of space/s.  

if we don't want to take the throughput matching route, then what do you do. At any point, we can calculate the responsetime. Given the response time, 

what if we try to minimize the slack in space and time and use that as the way to determine knob values. 
what is slack in space.the smallest precision with which we can navigate the space with. slack in space will determine the map resolution and slack in time to determine the volume commmunicated and number of iterations. note that 


how do you explain knobs? In other words, 1. why did we choose these knobs? 
Can I categorize the above knobs as intra and extra system? no, because 



I do think, we should take a cyber-physical codesign approach here. The idea is that given the related
Slack (in space and time) and 
 
note that a design which imposes very high resolution, is gonna have very small slack in time (since the velocity is so small to begin with), but very bad slack in space.   


space slack: The difference between the maximum space representation (voxel size) that a task need to maintain and how much its current representation. 
(it's really free space (corresponding to more accurate voxels) - free space( corresponding to less accurate map).
This is task dependent, but it's measured in volume, similar to the time slack that is task dependent but always measured in time.
how to calculate the space slack: fore

but we can easily compute how much time we need to spend to consume a volume of space. how? we know the volume, we know the resolution and we should have a model that tells us how much time is needed for a space with a certain volume and space. 

The problem with space


==> tex/dep/MAVBench-software-vulnerability.tex <==
\section{MAVBench soft-error Vulnerability} \label{sec:MAVBench-soft-error-vulnerability} 
In this section, we discuss our adopted error model and our error injection methodology. Then, we examine the impact of errors on MAVBench kernels and their propagation through out the end-to-end applications such as package delivery, search and rescue, etc. Various metrics such as functionality, performance and energy are used towards a thorough quantification of this impact. Furthermore, in order to understand the vulnerability cause, we profile the instruction mix and expose a correlation.   


\subsection{Error Model}

\subsection{soft error injection methodology}

\subsection{Vulnerability Quantification}


\subsection{Vulnerability cause}




==> tex/dep/characterization.tex <==
\begin{comment}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figs/slam-speed-energy.png}
\caption{relationship between drone's speed compute power}
\label{sec:powerbreakdown}
\end{figure}
\end{comment}
\begin{comment}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figs/desktop_vs_tx2_mapping.png}
\caption{relationship between motion planning performance and compute power}
\label{microbenchmark_1}
\end{figure}
\end{comment}
\section{The Role of Compute in MAVs}
\label{sec:char}

In this section, we discuss how compute affects MAV systems. At the high level, compute plays a crucial role both in the overall mission time and total energy consumption of such systems. First, we discuss each effect by providing relevant  theoretical background and supplement the discussion with a microbenchmark. Then, we analyze MAVBench as a set of representative applications in which such effects can manifest.   %Figure~\ref{fig:benchmarks_data_flow} and our benchmark suits and  discuss the high level insights into aerial agents bottlenecks and their corresponding implications. 


%thout the loss of generality we use our benchmark suit to conduct studies. The results and the flow presented in section blah to explain the corresponding  the by a discussion of  total system, i.e. locomotion and compute energy consumption, and its distribution. Then, we provide case studies showing that more compute can result in an improvement in the overall system's energy consumption. Finally we delve into our application benchmark suit to discuss how such a role can effect them.

%\subsection{Compute and Accuracy Relationship}
%explain slam and present the microbenchmark

\subsection{Compute and Flight Time Relationship}

Compute can play an important role in reducing the drone's mission time by increasing the mission's average velocity. Concretely, we identify that the reduction in hover time and the increase in maximum allowed velocity are the two major ways with which more compute can contribute to a higher average velocity. Here, we shed light on these different ways.

\paragraph{Hover Time Reduction:} Hover time and the average velocity have an inverse relationship, namely, the more drone spends time on hovering, the lower its average velocity. Similar to an idling CPU, a hovering drone is unfavorable since it is not working toward its mission, but yet wasting its limited energy. A hovering drone typically is waiting for its mission planning stage to make a decision (e.g. deciding on a path to follow). \emph{More compute power can help reduce hovering (e.g by reducing the decision making time),} hence decreasing the negative effect hovering has on the average velocity. 
\begin{figure}[t!]
\centering
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/fig_13}
    \caption{Theoretical max velocity.}
    \label{fig:process-time-velocity}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
    \centering
   \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/slam_fps_velocity_energy}
    \caption{Measured max velocity.}
    \label{fig:slam-velocity-energy}
    \end{subfigure}
\vspace{-5pt}
%\setlength{\belowcaptionskip}{-4ex}
\caption{\emph{(a)} Theoretical relationship between processing time and maximum velocity. \emph{(b}) Relationship between SLAM throughput (FPS) and maximum velocity and energy of UAVs.}
%\label{SOLO_power_breakdown}
\end{figure}

\paragraph{Max Velocity Increase, Collision Avoidance Effect:} The maximum velocity of the drone is not only mechanically bounded, but also compute bounded. For a given flight velocity, a collision-free flight is only possible if the drone can process its surrounding fast enough to react to it. Therefore, \emph{a higher velocity requires a faster processing capability}. The collision avoidance task can be rather compute intensive exercising various stages of the pipeline starting from the pixel processing in the perception stage and ending with the command issue in control. In order to guarantee collision avoidance, a  drone's maximum velocity is determined based on the aforementioned pixel to response time. Equation~\ref{eq:runtime-compute-bound} specifies the components involved in setting this velocity where $\delta_{t}$, d, $a_{max}$ and v denote process time, required stopping distance, maximum acceleration limit of the drone and maximum velocity~\cite{high-speed-nav}. As \Fig{fig:process-time-velocity} shows, our simulated drone, in theory, is bounded by the max velocity anywhere between 8.83 to 1.57 m/s given a pixel to response time of the range 0 to 4~seconds. 

\begin{comment}
\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs/fig_13}
\caption{Theoretical relationship between process time and max velocity}
\label{sec:vel_proc_relationship_figure}
\end{figure}
\end{comment}

\begin{equation}
\label{eq:runtime-compute-bound}
v_{max} = a_{max}(~\sqrt[]{\delta{t}^2 + 2\frac{d}{a_{max}}} - \delta{t})
\end{equation}
\setlength{\belowcaptionskip}{-1ex}

\paragraph{Max Velocity Increase, Localization Failure Effect:} The faster the speed of the drone, the higher the likelihood of its localization failure because the environment changes rapidly around a fast drone. Kernels such as SLAM which help localize the drone by tracking a set of points/features through successive camera frames struggle to keep up with the rate of these changes. It is important to note that localization failures can have catastrophic effects such as permanent loss or spending of extra time (for example by backtracking) for re-localization. 

Minimizing or avoiding localization related failure scenarios is highly favorable, if not necessary. To examine the relationship between the compute, maximum velocity and localization failure, we devised a micro-benchmark in which the drone was tasked to follow a predetermined circular path of the radius 25~meters. For the localization kernel, we used ORB-SLAM2 and to emulate different compute powers, we inserted a sleep in the kernel. We swept different velocities and sleep times and bounded the failure rate to 20\%. As \Fig{fig:slam-velocity-energy} shows, higher FPS values, i.e. more compute, allows for a higher maximum velocity for a bounded failure rate. 

%\begin{figure}[h]
%\includegraphics[]{figs/blank.pdf}
%\caption{Measurement set up to collect power data for 3DR Solo.}
%\label{sec:powerbreakdown}
%\end{figure}
\begin{figure}[!t]
\centering
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/power_break_down_tx2}
    \caption{Measured power breakdown.}
    \label{fig:SOLO-power-breakdown}
    \end{subfigure}
    \begin{subfigure}{.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=1.0\columnwidth]{figs/drone-power-time-series}
    \caption{Measured mission power.}
    \label{fig:drone-power-time-series}
    \end{subfigure}
\caption{\emph{(a)} Measured power consumption of a flying 3DR Solo. \emph{(b)} Total measured power consumption while the drone is "Flying" at two different steady-state velocities. The power consumption is severely dominated by the quad rotors by 20X.}
\label{SOLO_power_breakdown}
\end{figure}
\subsection{Compute and Energy Relationship}
The compute subsystem can also have a significant role in reducing total MAV energy consumption. To understand this, first we present the power distribution associated with \solo~\cite{solo3DR}, a popular off-the-shelf MAV. To measure power, we attach a wattmeter known as Eagle~Tree Systems eLogger~V4~\cite{eLoggerV4} to the \solo's battery during flight. The wattmeter allows us to collect data over time at 50~Hz while the drone flies. We command the drone to fly for fifty seconds and pull the data off of the wattmeter after the drone lands.

% The wattmeter gave us the total power consumed by the drone, without a deeper breakdown. To estimate the portion of the instantaneous power that would typically be consumed by a MAV's processor, we subtracted the idle power consumption of the \solo's default on-board computer and added to it the power consumed by the TX2 during typical workloads.

As \Fig{SOLO_power_breakdown} shows, the majority of the power consumption is dedicated to rotors (locomotion) and the compute only occupies a small portion of the entire pie and its role seemingly trivial. Although small in quantity, compute can have a grand effect on the system's power. This is because by reducing the mission time (as explained in the previous section), more compute power can, in fact, reduce the bigger portion of the pie, namely rotors energy consumption (due to a shorter flight). Note that although more compute can lead to more energy consumption of the compute subsystem, the reduction in rotor's energy can easily outweigh such an increase.  
% \setlength{\belowcaptionskip}{-2ex}


We profiled the mission time and the energy associated with the aforementioned microbenchmark. As the bottom plot in \Fig{fig:slam-velocity-energy} shows, higher compute capability results in increased SLAM FPS and hence a reduction in mission time by allowing for faster velocity. The reduced mission results in reduced total system energy, as the top plot in \Fig{fig:slam-velocity-energy} shows. By increasing processing speed by 5X, we were able to reduce the drone's energy consumption by close to 4X.

\subsection{MAVBench Workloads Compute vs. Flight Time vs. Energy}
\label{sec:operating-spoints}
We use our benchmark suite as a representative set of applications to examine the effect of compute on MAV systems. To analyze this effect, we conducted sensitivity analysis to core and frequency scaling of the TX2 board. TX2 has two sets of cores, namely a \textit{HMP Dual Denver cores} and a \textit{Quad ARM A57}. We turned off the Denver cores so that the indeterminism caused by process to core mapping variations across runs would not affect our results.
Average velocity, mission, and energy values of various operating points are profiled and presented as heat maps (\Fig{fig:benchmarks:OPA:scanning}---\Fig{fig:benchmarks:OPA:ap}) for a DJI Matrice 100 drone. \emph{In general, compute can improve mission time and lower energy consumption by as much as 5X.}

\paragraph{Scanning:}
We observe trivial differences for velocity, endurance and energy across all three operating points (\Fig{fig:benchmarks:OPA:scanning:velocity}, \Fig{fig:benchmarks:OPA:scanning:time}, and \Fig{fig:benchmarks:OPA:scanning:energy}). This is despite seeing a 3X boost in the motion planning kernel, i.e. lawn mower planning, which is its bottleneck (\Fig{fig:kernel-breakdown}). The trivial effect of compute on this application is because planning is done once at the beginning of the mission and its overhead is amortized over the rest of the mission time. For example the overhead of planning for a 5 minute flight is less than .001\%.  
%\vspace{2pt}

%We present our understanding and takeaways regarding the computational bottlenecks and the effect of compute on them.


%Each application and its associated nodes are time profiled (table~\ref{kernel_makeup}).  We use this table along with the data flow presented in figure    \label{fig:benchmarks} to dissect and understand various compute bottlenecks. 

%At the high level, each application contains a node called mission planner responsible for high level decision making and arbitrating flight command issuance. When needed, this nodes place a service call to the motion planning kernel, setting out drones next set of moves. Some of our applications have the collision avoidance capability. This node exercises all stages of the pipeline starting from the perception stage, i.e. point cloud generation, OctoMap, collision check, to planning, mission planner/motion planner and ending with control, i.e. path tracking/command issue. 

 
%and their kernel makeup is provided. This will help us to understand the bottle-necks and opportunities for improvements.

%It would be wise to note that this application is intentionally design minimally without an involved perception and planning because ~\red{ask vijay. He knows very well how to justify this}.

\paragraph{Package Delivery}:  As compute scales with the number of cores and/or frequency values, we observe a reduction of up to 84\% and 82\% for the mission time and energy consumption, respectively (\Fig{fig:benchmarks:OPA:pd:time}, and \Fig{fig:benchmarks:OPA:pd:energy}). The sequential bottlenecks i.e. motion planning and OctoMap generation kernel are sped up by frequency scaling to enable the observed improvements. There does not seem to be a clear trend with core scaling, concretely between 3 and 4 cores. We conducted investigation and determine that such anomalies are caused by the non-real-time aspects of ROS, AirSim and the TCP/IP protocol used for the communication between the companion computer and the host. We achieve up to 2.9X improvement in OctoMap generation and that leads to maximum velocity improvement. It is important to note that although we also gain up to 9.2X improvements for the motion planning kernel, the low number of re-plannings and its short computation time relative to the entire mission time render its impact trivial. Overall the aforementioned improvements translate to up to 4.8X improvement in the average velocity. Therefore, mission time and the MAV's total energy consumption are reduced.

%OctoMap generation is a major computationally intensive kernel in this application. This kernels performance OctoMap is of utmost importance since it is on the collision avoidance path. As shown in the data flow, this path starts with depth images and flows through point cloud generation, OctoMap generation, collision check and finally ends in the control.  OctoMap is responsible for 99\% of the pixel to response time determined by this path. Figure blah shows how OctoMap kernel scales with different number of cores and frequencies. 

%Motion planner is another computationally intensive kernel for this application. Although at first glance, its optimization can improve the mission time, the low number of re-plannings and its short computation time relative to the entire mission time render its impact trivial. For example, if we re-plan 20 times during the coarse of 5 minutes of the mission time, planning time would only consume .01\% of the entire flight.  
 
\begin{comment}
\begin{figure}[h]
\includegraphics[width=\columnwidth]{figs/velocity_process_time_relationship}
\caption{Theoretical relationship between process time and max velocity}
\label{sec:vel_proc_relationship}
\end{figure}
\end{comment}

%lowering the process time, results in a higher velocity and in turn, lowering the mission time and energy. 
%Explain collision avoidance path and policty and then discuss how octomap and planning comprise most of the it and the rest is ros runtime overhead. 
%Our pixel to response time is equal to 1.2 seconds most of which is dedicated to octomap and planning as is showing in the table.   

%As opposed to the surveying benchmark, package delivery's trajectory is determined at the mission time.  perception of the obstacles surrounding the drone at any moment and also on the way to the destination is required. To do so, a map of once visible and visited environment is created and maintained within an octomap structure \ref{blah}. Arriving at such a map requires converting image depth information to point clouds (point cloud generation node) and integrating them to the map (octomap server). It is important to note the dynamic obstacles are intentional not captured within the octomap. Motion planner, attempts to find the shortest path to the destination with the knowledge of such map and only remap on demand. 
  
%As the drone follow its trajectory, new trajectory can be demanded due to environmental triggers. These environmental triggers can be static obstacles unaccounted for at the time of planning (since they were not in the sensor's visibility range). Dynamic obstacles not present at the time of planning can also trigger replannings. 

%These triggers are identified using the panic and the future collision node. The future collision node identifies whether an obstacle (mainly static ones) is on the trajectory planned and alarm the mission planner node to request a re-plan. Since future collision operates on octomap, dynamic obstacles can not be spotted to be reacted to. This is an intentional decision since dynamic obstacles can move out of the path.
%Panic node, alarms the drone of any obstacles that enters a virtual halo surrounding the drone by processing the point cloud. By equipping the drone with a forward and backward camera, we can avoid most obstacles\footnote{since each camera only has a FOV of 120 degree, there are blind spots for our drone. To fix this, more sensors are required. We address this issue in the limitation section}  This node is our solution to dynamic obstacles. In addition to dynamic obstacles, this node can save the drone from crashing in any obstacle if the control node (follow trajectory) allows for a drift from it's supposed trajectory. 

%Due to small number of replannings, the hover time associated with the planning stage has a minor affect on the mission time. In addition, small time associated with real time threads such as panic and future collision does not demand more attention. Hence, compute's role on this application is minor.

{
\begin{figure}[t!]
    	\centering
    	\begin{subfigure}[t!]{.3\columnwidth}
    	\centering
    		\includegraphics[width=\columnwidth]{figs/scanning_velocity_operating_point}
    		\caption{Velocity (m/s)}
            \label{fig:benchmarks:OPA:scanning:velocity}
    	\end{subfigure}
        \begin{subfigure}[t!]{.3\columnwidth}
    	\centering 
    \includegraphics[width=\columnwidth]{figs/scanning_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:scanning:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/scanning_energy_operating_point}
    \caption{Energy (kJ)}
    \label{fig:benchmarks:OPA:scanning:energy}
    \end{subfigure}
    \caption{Scanning.}
    \label{fig:benchmarks:OPA:scanning}
    \end{figure}%
   \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:pd:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/pd_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:pd:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/pd_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:pd:energy}
    \end{subfigure}
    \caption{Package Delivery.}
    \label{fig:benchmarks:OPA:pd}
    \end{figure}%
    \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:mapping:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/mapping_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:mapping:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/mapping_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:mapping:energy}
    \end{subfigure}
    \caption{Mapping.}
    \label{fig:benchmarks:OPA:mapping}
    \end{figure}%
    \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_velocity_operating_point}
    \caption{Velocity (m/s)}
     \label{fig:benchmarks:OPA:sar:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/SAR_flight_time_operating_point}
    \caption{Mission Time (s)}
    \label{fig:benchmarks:OPA:sar:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/SAR_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:sar:energy}
    \end{subfigure}
    \caption{Search and Rescue.}
    \label{fig:benchmarks:OPA:sar}
    \end{figure}
    \begin{figure}[t!]
    \centering
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_error_operating_point}
    \caption{Error Rate(m/s)}
     \label{fig:benchmarks:OPA:ap:velocity}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{figs/aerial_photography_flight_time_operating_point}
    \caption{Mission Time(s)}
    \label{fig:benchmarks:OPA:ap:time}
    \end{subfigure}
    \begin{subfigure}[t!]{.3\columnwidth}
    \centering
    \includegraphics[width=\columnwidth] {figs/aerial_photography_energy_operating_point}
    \caption{Energy (kJ)}
     \label{fig:benchmarks:OPA:ap:energy}
    \end{subfigure}
    \caption{Aerial Photography.}
    \label{fig:benchmarks:OPA:ap}
\end{figure}
}


\paragraph{Mapping:} We observe a reduction of up to 86\% and 83\% for the mission time and energy consumption, respectively, as compute scales with the number of cores and/or frequency values (\Fig{fig:benchmarks:OPA:mapping:velocity}, \Fig{fig:benchmarks:OPA:mapping:time}, and \Fig{fig:benchmarks:OPA:mapping:energy}). The concurrency present in this application (all nodes denoted by circles with a filled arrow connection or none at all in \Fig{fig:benchmarks:data-flow:mapping} run in parallel) justifies the performance boost from core scaling. The sequential bottlenecks, i.e. motion planning and OctoMap generation explains the frequency scaling improvements. We achieve up to 6.3X improvement in motion planning (\Fig{fig:kernel-breakdown}) and that leads to hover time reduction. We achieve a 6X improvement in OctoMap generation and that leads to maximum velocity improvement. The improvements translate to a 5.3X improvement in average velocity. Since mission time is reduced, total energy consumption reduces.


\paragraph{Search and Rescue:} We see a reduction of up to 67\% and 57\% for the mission time and the energy, respectively, as compute scales (\Fig{fig:benchmarks:OPA:sar:velocity}, \Fig{fig:benchmarks:OPA:sar:time}, and \Fig{fig:benchmarks:OPA:sar:energy}). Similar to mapping, more compute allows for the reduction of hover time and an increase in maximum velocity which contribute to the overall reduction in mission time and energy. In addition, a faster object detection kernel prevents the drone from missing sampled frames during any motion. We achieve up to 1.8X, 6.8X, and 6.6X speedup for the object detection, motion planning and OctoMap generation kernels, respectively. In aggregate, these improvements translate to 2.2X improvement in the MAV's average velocity.

\begin{comment}
\begin{figure}[!t]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=0.9\linewidth]{figs/tx2-desktop}
\vspace{-12pt}
\caption{Comparing a full-on-edge drone versus a full-on-cloud drone. Our system allows part or portion of the MAVBench workloads to be offloaded to the cloud (or another local co-processing agent).}
\label{fig:cloud_edge}
\end{figure}
\end{comment}

\paragraph{Aerial Photography:} We observe an improvement of up to 53\% and 267\% for \emph{error} and mission time, respectively (\Fig{fig:benchmarks:OPA:ap:velocity}, \Fig{fig:benchmarks:OPA:ap:time}, and  \Fig{fig:benchmarks:OPA:ap:energy}). In aerial photography, as compared to other applications, higher mission time is more desirable than a lower mission time. The drone only flies while it can track the person, hence a longer mission time means that the target has been tracked for a longer duration. In addition to maximizing the mission time, error minimization is also desirable for this application. We define error as the distance between the person's bounding box (provided by the detection kernel) center to the image frame center.  Clock and frequency improvements translate to 2.49X and 10X speedup for the detection and tracking kernels and that allows for longer tracking with a lower error. No significant trend is observed in the energy data because energy depends on both the mission time and the velocity, and as opposed to the other applications, there is no need for the drone to minimize its velocity. Instead, it needs to successfully track the person.


\begin{figure*}[!t]
\centering
\includegraphics[width=\columnwidth]{figs/kernel-breakdown_2}
\vspace{-18pt}
\caption{Kernel breakdown for MAVBench. The abbreviations are as follows: \emph{OD-}Object detection, \emph{MP-}Motion Planning, \emph{OMG-}OctoMap Generation for kernels and \emph{SC-}Scanning, \emph{PD-}Package Delivery,  \emph{MAP-}3D Mapping, \emph{SAR-}Search and Rescue, and \emph{AP-}Aerial Photography for applications. The $x$-axis lists the kernel-application names and $y$-Axis represents the runtime in seconds. Each bar graph represents one of the configurations used in the hardware. The cores are varied from 2 to 4 and the frequency goes from from 0.8 GHz , 1.5 GHz or 2.2 GHz.}
\label{fig:kernel-breakdown}
\end{figure*}

%\begin{minipage}[!]{0.99\columnwidth}
   
%\end{minipage}


%In the perception stage of this application, a person is detected, and the bounding box associated with the person is tracked. The tracking stage consists of two nodes itself. The first node (buffer then track) buffers the images while detection is running and then track the buffered once the person is detected. The second node (track continuously) tracks the previous bounding box while the new one is calculated. Buffer then track node is necessary, since otherwise, image difference between the image detection sampled and tracking is large enough that increases the false positive tracking. PID node calculates the difference between the targets place and where it should be in the frame and sends small trajectories to the drone. Similar to other applications, these trajectories are followed in the follow trajectory node.

%Compute's effect on this application is on its accuracy and the duration in which drone can follow the target. In other words, faster compute can affect how closely and for how long the target is tracked. 
%\subsection{Understanding the Compute to Endurance Relationship}
%in this section, we demonstrate the relationship between compute on the drone and the drone's mission time (i.e., endurance). We start by showing that looking naively indicates that compute consumes an insignificant amount of power, and that much of the power is spent on keeping the drone afloat using its rotors. Therefore, this leads to a shortsighted conclusion that compute does not play a dominant role in autonomous flight for dron

%\subsection{Micro architectural characterization}
%To understand the reason behind the aforementioned bottlenecks, we provide micro-architectural characterization of them. This will help the designers to design for the future MAV systems while alleviating such bottlenecks. Our analysis show that the bottle necks mainly exists in the perception and the planning stage. Hence, we turn our focus solely to these two stages.  
%
%characterize OctoMap, slam and nbvPlanner. 

\begin{comment}
%\subsubsection{Algorithmic Choices}
%Algorithms at some point will be general enough to cover all the environments, hence we shouldn't 
%be highlighting our algorithmic sensitivity to environment (which in this argument is considered in a flaw)
 
\subsection{explanation of each apps inter kernel interactions}
\textbf{Scanning:} This application involves only a single ROS node. All the code runs on a CPU, with no parallelization. The main computational kernel is the simple path-planning since no collision-checking is involved. This is because the \textit{Scanning} benchmark is meant for outdoors environments, high aboveground where obstacles are not to be found. Because the benchmark is meant for outdoors environments, localization is accomplished through the use of GPS sensors, which incur negligible computational overhead.

\textbf{Aerial Photography}
This application involves three ROS nodes running concurrently. One node is responsible for running object detection algorithms to locate the human target. However, object detection is normally a very computationally-intensive task that can take up to several seconds to complete. Therefore, another node runs much faster tracking algorithms such as KCF which estimate the position of the target in the interval between completions of the object detection algorithm. Another node controls the motion of the MAV based on the position of the target. All nodes run on the CPU except for the object detection node which runs on a GPU.

\textbf{Package delivery:}
This application involves 4 ROS nodes, which all run on CPU cores. One node plans collision-free trajectories using the path-planning algorithms described in the previous section. Another node waits for paths to be planned and then controls the motion of the MAV to follow them. However, as the MAV follows these trajectories, it may uncover new obstacles in its environment that had been out of range of its sensors when the path was initially planned. Therefore, an additional node must constantly run to check whether any newly uncovered obstacle causes a collision upon the planned trajectory, so that the path can be re-planned if necessary. Finally one final node must provide localization capabilities, either through GPS or SLAM, to enable the MAV to follow its planned trajectory accurately.

\textbf{Mapping}
This application involves 3 ROS nodes which all run on CPU cores. One node samples its environment and finds points on the boundary of previously explored space where the MAV can be expected to maximize the amount of unknown space that it uncovers. Once these points are found, the node then plans a path towards them along an RRT tree. A second node controls the motion of the MAV, following the trajectories generated by the first node. Finally, a third node must provide localization, such as through SLAM. This localization must be accurate, because the MAV updates its internal map based upon the position it believes it is in. If the MAV relies upon an inaccurate SLAM algorithm, the map it generates may not be completely accurate.


\textbf{Exploration:}
Computationally, this application includes the same nodes as the \textit{Exploration} benchmark, as well as another node that constantly runs object detection algorithms to search for human victims as it explores unknown environments. The object detection node here runs on a GPU. The object detection algorithm must run fast, in order to allow the MAV to sweep a large area quickly, but they must also be highly accurate, to prevent the MAV from missing a victim due to a false negative.


\label{sec:characterization}
 possibly the bottlenecks, and a table with kernel times and their distribution.
 
 possibly the requirements compute wise and which platforms are suitable for them (refer back to the HIL and how we can conduct these conclusive studies)

\subsection{Environment and it's effects}
indoor/outdoor,
obstacle density, dynamic obstacle speed
\subsection{}

\end{comment}

 


==> tex/dep/diff.tex <==
%DIF < \section{Compute-driven, Flight-Efficiency Optimization: A Case Study}
\section{\DIFaddbegin \DIFadd{Compute-driven, Flight-Efficiency Optimization: A }\DIFaddend Case \DIFdelbegin \DIFdel{Studies}\DIFdelend \DIFaddbegin \DIFadd{Study}\DIFaddend }
\label{sec:case-study}

Our closed-loop simulation platform, together with our plug and play benchmarks, enables a holistic inspection of intra-system and system/environment interactions. Studying of the former open doors for hardware/software co-design studies. Such studies starts with the profiling and sensitivity analysis as exemplified in the previous section. The latter enables environment focused considerations and designs such \DIFdelbegin \DIFdel{as reliability studies%DIF < , i.e. the effect of various localization kernels and collision avoidance algorithms on the system. 
}\DIFdelend \DIFaddbegin \DIFadd{reliability studies, i.e. the effect of various localization kernels and collision avoidance algorithms on the system. }\DIFaddend In this section \DIFdelbegin \DIFdel{, we conduct performance, energy and reliability case studies  highlighting the insights architects can take advantage of by using our platform.   
}%DIFDELCMD < \red{\subsection{Sensor-cloud: A Performance Case-Study}
%DIFDELCMD < As opposed to the studies provided in the previous section where our setup emulated a fully-on-edge drone (i.e. a drone which all of its computation is done on the drone itself), our setup can further examine a cloud/edge drone where the computation is distributed across the edge and the cloud. To examine the impact of cloud computing for MAVs, we compare a fully-on-edge drone equipped with a TX2 versus a fully-in-cloud drone with only a minimal computer on board (i.e. a flight controller) but a powerful cloud support (mention the x86 platform we used). This case study targets Mapping as the application of choice. As can be seen in Fig.\ref{fig:edge_cloud}, a drone that can enjoy the cloud's extra compute power sees a 3X speed up in planning time. This improves the average velocity of the drone due to the reduction in hover time and hence reduces the overall mission time almost to half.
%DIFDELCMD < }
%DIFDELCMD < \begin{figure}[t!]
%DIFDELCMD < \centering
%DIFDELCMD < \includegraphics[trim=0 0 0 -25, clip, width=0.9\linewidth]{figs/tx2-desktop}
%DIFDELCMD < %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{Comparing a full-on-edge drone vs a full-on-cloud drone.}}
%DIFAUXCMD
%DIFDELCMD < \label{fig:cloud_edge}
%DIFDELCMD < \end{figure}
%DIFDELCMD < %%%
\subsection{\DIFdel{Environment Aware Design: An Energy Case-Study}}  
%DIFAUXCMD
\addtocounter{subsection}{-1}%DIFAUXCMD
\DIFdelend \DIFaddbegin \DIFadd{we consider an example of the latter.   
}

\DIFaddend We conduct a kernel/environment sensitivity analysis using the OctoMap node~\cite{octomap}, which is a major bottleneck in \DIFdelbegin \DIFdel{3 of our end to  applications, namely package package delivery, mapping and search and rescue}\DIFdelend \DIFaddbegin \DIFadd{our benchmark suite}\DIFaddend . OctoMap is used for modeling of various environments without prior assumptions. In order to do so, the map of the environment is maintained in an efficient tree-like data structure while keeping track of the free, occupied and unknown areas. Both planning and collision avoidance kernels utilize this data structure to make safe flights possible by only allowing the drone to navigate through free spaces.  

\DIFdelbegin %DIFDELCMD < \begin{figure}[b]
%DIFDELCMD < \centering
%DIFDELCMD < \includegraphics[trim=0 0 0 -25, clip, width=\columnwidth]{figs/octomap_resolution_with_boxes}
%DIFDELCMD < %%%
%DIF < \vspace{-30pt}
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{OctoMap accuracy (resolution) versus performance.}}
%DIFAUXCMD
%DIFDELCMD < \label{fig:octrest}
%DIFDELCMD < \end{figure}
%DIFDELCMD < 

%DIFDELCMD < \begin{figure*}[t!]
%DIFDELCMD <     \centering
%DIFDELCMD <     \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_sim}
%DIFDELCMD <        \vspace{-30pt}
%DIFDELCMD <         %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{Environment's Map}}%DIFAUXCMD
%DIF < Level-1 Evaluation}
         %DIFDELCMD < 

%DIFDELCMD <         %DIFDELCMD < \label{fig:game:level-1}%%%
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <     \hfill
%DIFDELCMD <     \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_rviz__15}
%DIFDELCMD <        \vspace{-30pt}
%DIFDELCMD <        %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{resolution of .15 }\emph{\DIFdelFL{(m)}}%DIFAUXCMD
}
        %DIFAUXCMD
%DIFDELCMD < \label{fig:rviz__15}
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <     \hfill
%DIFDELCMD <      \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_rviz__5}
%DIFDELCMD <        \vspace{-30pt}
%DIFDELCMD <        %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{resolution of .5 }\emph{\DIFdelFL{(m)}}%DIFAUXCMD
}
        %DIFAUXCMD
%DIFDELCMD < \label{fig:game:rviz__5}
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <        \hfill
%DIFDELCMD <    \begin{subfigure}{.23\linewidth}
%DIFDELCMD <         \centering
%DIFDELCMD <         \includegraphics[trim=0 -10 0 -10, clip, width=\textwidth]{figs/garage_rviz_1}
%DIFDELCMD <         \vspace{-30pt}
%DIFDELCMD <         %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
\DIFdelFL{resolution of .8 }\emph{\DIFdelFL{(m)}}%DIFAUXCMD
}%DIFAUXCMD
%DIF < Level-3 Evaluation}
        %DIFDELCMD < \label{fig:game:rviz_1}
%DIFDELCMD <     \end{subfigure}
%DIFDELCMD <     \hfill
%DIFDELCMD <    \vspace{+30pt}
%DIFDELCMD <    %%%
%DIFDELCMD < \caption{%
{%DIFAUXCMD
%DIFDELCMD < \small %%%
\DIFdelFL{Drone's environement }\emph{\DIFdelFL{(a)}} %DIFAUXCMD
\DIFdelFL{and its perception of it with various OctoMap resolutions (}\emph{\DIFdelFL{(b)}}%DIFAUXCMD
\DIFdelFL{, }\emph{\DIFdelFL{c}}%DIFAUXCMD
\DIFdelFL{, emph}%DIFDELCMD < {%%%
\DIFdelFL{d}%DIFDELCMD < }%%%
\DIFdelFL{).}}
    %DIFAUXCMD
%DIFDELCMD < \label{fig:octomap_perception}
%DIFDELCMD < \end{figure*}
%DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend % Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\vspace*{7pt}
\centering
\caption{Switching between OctoMap resolutions dynamically leads to mission success compared to 0.8~cm, and compared to 0.15~cm we consume less energy and thus retain more battery.}
\label{tbl:octopt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|l|l|l|}
\cline{2-4}
                                                                 & \textbf{Resolution {(cm)}}       & \textbf{Mission Status} & \textbf{Battery  (\%)} \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Package Delivery}}} & \textit{0.8}              & \cellcolor{red!25}Fail                    &   0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    &    81.00          \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    &   \cellcolor{green!25}86.00           \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Mapping}}}          & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0           \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 39.03        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}53.83        \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\textbf{Search and Rescue}}}              & \textit{0.8}              & \cellcolor{red!25}Fail                    & 0         \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{0.15}             & Pass                    & 24.21        \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                           & \textit{Chameleon (0.8, 0.15)} & Pass                    & \cellcolor{green!25}57.87        \\ \hline
\end{tabular}
}
\end{table}

Size of the voxels, i.e. the map's resolution, trades off accuracy and flight-time/energy. By lowering the resolution, i.e. increasing voxel sizes, obstacle boundaries get inflated, hence the drones perception of the environment and the objects within it becomes inaccurate. However, doing so improves the performance of the OctoMap node and eventually leads to a faster flight time. To examine the trade off, we ran OctoMap with various resolutions.
\DIFdelbegin %DIFDELCMD < \Fig{fig:octrest} %%%
\DIFdel{shows 4.5X speed up in the OctoMap's update rate for 6.5X reduction in accuracy. 
%DIF < \begin{comment}
}%DIFDELCMD < 

%DIFDELCMD < %%%
%DIF < \end{comment}
\DIFdelend %DIF > \Fig{fig:octrest} shows 4.5X speed up in the OctoMap's update rate for 6.5X reduction in accuracy. 
\DIFaddbegin \begin{comment}
\begin{figure}[b]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=\columnwidth]{figs/octomap_resolution_case_study}
\caption{OctoMap accuracy (resolution) versus performance.}
\label{fig:octrest}
\end{figure}
\end{comment}
\DIFaddend Certain aspects of the environment such as obstacle density determine the OctoMap resolution. In low density environments, where the drone has ample opportunities for paths to take, a low resolution can suffice. However, in dense environments, low resolutions can deprive the drone from path opportunities present since the drone perceive the obstacles bigger than they are. \DIFdelbegin %DIFDELCMD < \red{The impact of OctoMap resolution on the drone's perception can be easily seen in figure blah, where figure blah-1 shows the environment and the figure blah-2 through 4 show the drone's perception of the environment. As observed, when the resolution is lowered, the voxel sizes increase to the point that the drone can fail to recognize openings as possible passage ways to plan through. This in turn can result in a mission inefficiency and possible failures depending on the environment}%%%
\DIFdel{.
}\DIFdelend Since the environment around the drone changes, a dynamic approach where the resolution is set on the runtime is desirable. We study two environments during the mission, namely outdoors (low obstacle density) and indoors (high obstacle density). 

Table~\ref{tbl:octopt} shows the result of two static (predetermined) resolutions, 15~cm and 80~cm, and our proposed dynamic approach (Chameleon) that multiplexes between the two appropriately. The dynamic approach allows for up to 2.3X improvement in endurance. As compute reduces, OctoMap bottleneck eases, and therefore the drone completes its mission faster. 

The table also highlights another interesting relationship. Statically choosing the 80~cm resolution to optimize for compute (only) causes the drone to fail its mission since it is unable to plan paths through narrow openings in the indoor environments. By switching between two resolutions according to the environments obstacle density, Chameleon is able to balance OctoMap computation with mission feasibility and energy, holistically. Therefore, in all cases, Chameleon uses less energy and retains more battery charge. \DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < \red{\subsection{Depth Sensor Noise: A Reliability Case-Study}}
%DIFDELCMD < \red{Vijay could you add the information flow introduction you mentioned.}
%DIFDELCMD < 

%DIFDELCMD < \red{In this case study we examined the impact of sensor noise on the performance of our package delivery application. We injected Gaussian noise with a range of standard deviations into the depth readings of the drone's RGBD camera. Sensory noise distorts the drone's perception of the obstacles in its environment, and we found that Gaussian noise in particular \emph{inflates} obstacles, making them appear larger than they actually are. This causes the drone to re-plan its trajectories more often, as it assumes that its planned path will collide into objects that are actually further away than they seem, as shown in figure blah. The more the drone re-plans its paths, the longer it takes to reach its destination, increasing mission time by blah percent.
%DIFDELCMD < }
%DIFDELCMD <  %%%
\DIFdelend

==> tex/dep/dynamic_design_re_org.tex <==
\section{Dynamic world, Dynamic Design}
\label{sec:dynamic design}
To address the shortcomings associated with static designs, we present \texit{roborun}, a dynamic runtime solution. 
At the highlevel, roborun continoully monitors the backend to quantify the velocity
imposed deadline. Then, it adjusts the front-end imposed computational load to meet and further track the deadline closely. 
Note that since the spatial reasoning associated computation is distributed across perception and
planning stages, our runtime controls the computational payload within and across these stages. Doing so improves designs dynamicity and hence optimality.  
In this section, we discuss our runtime implementation. First, we present its overall arthictecture, and then, its
components in details.

\subsection{Overall Architecture}


\textbf{task graph perspective}
Our runtime, sits in sequence with the rest of the pipeline stages immdidately after the sensors (figure blah).
It uses a distributed design consisting of two main components, namely a governor, 
reponsible for determining the optimal policies, and a set of opertors, responsible for enforcing these policies.
At a highlevel, the governor continously profiles sensors to monitor variables such as velocity from the backend and depth image from the frontend. 
Using these information, it calculates the deadline and the computational load for various stages across the pipeline. 
It then uses its operators to enforce the computational load for each stage while meeting the end-to-end deadline.

\textbf{control-based formulation perspective}
Buidling on top of the successes of the control theory field, our runtime uses feed-forward/feedback based implementation (figure blah).
The feed forward path adjusts the load according to the current needs. 
To do so, it uses system's behavior models to simulate the impact of various computation loads, 
searches through the design space in realtime and find the most optimal load across different stages 
while meeting the required deadline. 

The feedback path improves the runtime accuracy by monitoring and learning from previous iterations' inefficiency.
This path \red{fill once the feed back path is developed more}

\subsection{Components: operators}
Operators are responsible for enforcing the policies, i.e., the knob settings decided by the governor. At the highlevel, each operator consists of a sequencer and a monitor/estimator. Our operators
either control the space precision or volume. Since the computation associated with spatial reasoning is 
distributed across the perception and planning stage, our operators augment both these stages and further 
the communication between the two. Table blah shows the list of our operators and their description. 

\subsubsection{Precision Operators}
There are total of two precision opertors. One controling the precision with which new point cloud is 
integrated into the map, and the other the precision within of the map which the planner explores.
The first one is enabled by controling the sampling rate of the points within the pointcloud.
The second is enabled by taking advantage of the inherent multi-resolution capability of the occupancy map
used.

\subsubsection{Volume Operators}
There are total of three volume operators, controlling the space volume integrated into the map per iteration,
the potential volume of space that the planner can plan through and finally the accumulated volume of space planner
get to plan through. All of our volume controllers consist of two components, namely a squencer and monitor. 
\textbf{Sequencer:} This block is responsible for prioretizing and further orchestrating the order with wich the space will be consumed. 
\textbf{Monitor}: This block is responsible for monitoring space volume size. 
The monitor screens the size of the volume that is being released by the sequencer. As the size reaches a threshold
decided by the governor, the monitor signals a termination to the sequencer stoping the consumption of space. 

Here we dicuss the priority policies and their implementation.  \red{I am not sure how to do this.
It just seems like we are too deep in the organizational hierarchy} 


\subsection{Components: governor}


\subsubsection{solver}
We formulate this problem as a optimization problem. 

\textbf{objective function}

\blueDebug{talk about why the objective function is setup the way it is} 
Equation blah shows the objective function and the constraints. 
The objective function is presented in equation blah, where delta denotes blah ... \red{go over the notation} 
Each one of the delta denote the performance models illustrating the relationship between, space precision, volume and latency.

\blueDebug{talk about how models are collected}Each one of these models are collected through having the drone to fly through various environment.



\textbf{constraints}
Equations blah through blah list our equality and inequality constraints. 



==> tex/dep/dynamic_world.tex <==
%\section{Compute vs. Flight-time vs. Energy Efficiency}
\subsection{Dynamic Demands of a Dynamic World}
\if\briefmode1
  \begin{briefenv} 
    \brief{Detail world's dynamicity sources and impact.}

- Dynamic frontend causing dynamic payload.

\hspace{3ex} - Dynamic space volume (des and quant).

\hspace{3ex} - Dynamic space precision (des and quant).

- Dynamic backend causing dynamic deadlines.

\hspace{3ex} - Dynamic velocity des and quant).
\end{briefenv}
\else
Cyber system of a robot is embedded in a dynamic framework which imposes varying computational demands. On the one hand, pipeline's front end, i.e., environment plus sensors, imposes  a changing
computational payload, and on the other, the backend, i.e., environement plus actuators, imposes a varying deadline. Sitting in the middle, compute absorbs such dynamics. In this section, first, we
detail the source of such dynamicity, and then, we quantify these variations. 


\textbf{Dynamic Frontend Means Dynamic Payload:} Navigation pipeline front end, i.e., environment plus the sensors, determine the computaional load, i.e, the amount of input data to be consumed. Events in the environments are captured through sensors and presented to the cybersystem for interpretation. The richer the environment and the higher the sensory samples, the higher the computational load. 


Since spatial reasoning sits at the heart of navigation, we consider space as the main processing payload, and further, identify \textit{volume} and \textit{precision} of space as two major drivers of the payload intensity.

\textit{
space precision:} space precision, i.e., the accuracy with which space is encoded, has a direct relationship with computational load. Increasing the precision, increases the number voxels that both the mapping and planning need to processes. This in turn increases the latency associated with the pipeline. Figure blah shows the relationship between, precision, number of voxels consumed by the mapping stage. As shown, an 2x increase in precision has a blahx increase in number of voxels.

Space precision should be dynamically determined based on robots surrounding environment properties. Environment congestion is an example of such determinant. Intuitively speaking, space with higher congestion requires a finer grain encoding so as to allow for seeing free spaces. Since such congestion varies throughout the mission, identifying and adapting the precision and hence the load accordingly is demanded. 

Figure blah depicts the dynamic nature of congestion and the corresponding payload. As the drone traverse an area, this congestion varies and so does with it the payload. As shown, a blahx increase in congetion causes an blahx increase in payload. As seen, for this flight, we observe a standard deviation of blah for the precision.
Note that we use average (or wosecase) gap size as the estimation of the congestion. 

\textit{Space Volume:} the volume of space processed at a time has a direct relationship with the computation load. The higher the volume, the higher the number of voxels consumed by the pipeline (Figure blah). This in turn increases the latency. Figure blah shows the relationship between, volume, and the number of voxels consumed by the mapping stage. As shown, an 2x increase in volume has a blahx increase in number of voxels.

Space Volume  dynamically changes based on environmental factors such as occlusion. Intuitively speaking, a robot whose vision is considerably blocked from different directions consumes less volume than a robot surrounded by free space. Figure blah depicts the dynamic nature of volume. As our drone traverse an area, it is occluded at different times with different intensity and so does with it the payload. As seen, for this flight, we observe a standard deviation of blah for the volume.




\textbf{Dynamic Backend Means Dynamic Deadline:} Navigation pipeline backend, i.e., the environment and the acutation determine the compute deadline. Intuitively speaking, as the robot's speed increases, it needs to react to its surroundings faster. This in turn demands faster decision making, and hence lower deadlines per decision. Figure blah depicts this relationship. The data presents the time sequence of a drone's velocity which is tasked with reaching a destination in a collision-free flight. The redline shows how the time budget per iteration varies a function of robot's speed. As seen, we observe a standard deviation of blah x associated with velocity and blahx for deadline. 


\begin{comment}
In this section, we show how the dynamic nature of the systems that the compute subsystem of a robot interact with impose dynamic demands. A flexible compute subsystem is necessary to adapt to such demands. Concretley, we identify the external world and the other subsystems of the robot as the main agents of such dynamicity. 

maybe I can use the slacked caused by the change in velocity as 

can I show how the gap sizes change (we need to have som representable maps, or possibly mention some average values inside and outside, and then fill inthe values in between). Can we do the same thing with velocity? How about volume

surrounding the compute subsystemcompue subsystem of a robot is stressed with different level of serverity through out a mission. 


To motivate, in this section, can we just show all the slacks that are present, or possibly overutilization or underutilization caused.

for velocity, we can show the response time slack for a specific max velocity.

for gap sizes, we can show how much less time we can spend if we adjust (so the difference between time spend and the time needed)

how about volume?

can we use the possible velocity (given the response time) and the difference bteween possible velocity and actual velocity to show the inefficiency


In this section, first, we discuss the concept of bottleneck for a cyber-physical systems. Then, we propose a unifying metric across the entire robot complex to facilitate this identification. Then, we turn our focus to cyber system, describing how compute can improve the performance when it is not the bottleneck. 
\label{sec:dynamic world}

\subsection{Bottleneck Identification}
\label{sec:bottleneck_identification}
In a system, a component/kernel is identified as the bottleneck if its performance is worse than its predecessors and successors. Concretely, in a computing system, the bottleneck has  the lowest throughput. Bottleneck identification and relaxation is widely adopted within the computing community. For example, in a system with 3 chained accelerators, the accelerator with the least OPS is the bottleneck. Identifying the bottleneck requires defining common performance metrics, shared across all the system components, such that they can be compared against one another. In the cyberland, metrics that quantify the rate of information such as OPs, FLOPs, Byte/s, and etc are used. 

We need to find metrics that marry the physical and the cyber world to identify the bottleneck within a robot complex. This is because as opposed to the compute subsystem, performance metrics for non-cyber stages, such as sensors and actuators, measure physical quantities such as range, and velocity. Given the robot's continual interaction-with and further manipulation-of its surrounding space, we propose using 3d space volume as the quantity of interest. Consequently, we gauge performance by the rate with which robot's surrounding space is changed, captured, interpreted and reacted to.   

Since the producer/consumer computing system model, facilitates the identification of the bottleneck, we adopt a similar model for an entire robot complex. With space as the quantify of interest, producers generate the new space, and consumers interpret it. Figure below shows the role of each subsystem within this model. 
	As the drone moves around using its actuators, it is exposed to its surrounding space which is then captured using sensors (with certain range and fps). Sensors/actuator combo can become the bottleneck when the space captured by them is smaller than the space interpreted by the compute. Consider a sensor with the range of d. Uppon traversal of x meters (assuming no occlusion), the volume captured by the sensors are equal to x*pi*d**2, where x is vt. For compute to catch up volume interpreted by compute/per sec (i.e., pi*d**3*throughput) should be bigger than that presented by the actuator sensor combo. Occllusion and smaller velocity results in shifting the bottleneck from compute to the sensor/actuator combo.  In the case drone is flying full speed and has no occlusion, compute can become the bottleneck. 

In addition to interpreting the space, the robot needs to react to what happens in the space around it.  The actuators specifically can become the bottleneck when the Space uncovered and reacted to > space traversed (dd/dt which is v). Reaction is task specific. In this paper we target point to point navigation where the drone needs to react to the obstacle around it. In the worse case scenarios where is at full speed at a distance of d, the drone needs to stop before running into the obstacle. In the case in which the drone is not flying as fast, actuators and sensors can be the bottleneck. (Note that if we can make an argument for d as well, ie.., depending on d we should also set v, and we should be able to easily get d from piont cloud).  
ther manipulate their surrounding space, we propose using 3d space volume as the quantity of interest. Considering this metric, performance metrics can be defined as the rate with which space surrounding the robot changes (either due to the robot itself or other agent), and further rate with which such changes are captured, interpreted and reacted to.   
Since the producer/consumer computing system model, facilitates the identification of the bottleneck, we adopt a similar model for an entire robot complex. With space as the quantify of interest, producers generate the new space, and consumers interpret it. Figure below shows the role of each subsystem within this model. 
	As the drone moves around using its actuators, it is exposed to its surrounding space which is then captured using sensors (with certain range and fps). Sensors/actuator combo can become the bottleneck when the space captured by them is smaller than the space interpreted by the compute. Consider a sensor with the range of d. Uppon traversal of x meters (assuming no occlusion), the volume captured by the sensors are equal to x*pi*d**2, where x is vt. For compute to catch up volume interpreted by compute/per sec (i.e., pi*d**3*throughput) should be bigger than that presented by the actuator sensor combo. Occllusion and smaller velocity results in shifting the bottleneck from compute to the sensor/actuator combo.  In the case drone is flying full speed and has no occlusion, compute can become the bottleneck. 

In addition to interpreting the space, the robot needs to react to what happens in the space around it.  The actuators specifically can become the bottleneck when the Space uncovered and reacted to > space traversed (dd/dt which is v). Reaction is task specific. In this paper we target point to point navigation where the drone needs to react to the obstacle around it. In the worse case scenarios where is at full speed at a distance of d, the drone needs to stop before running into the obstacle. In the case in which the drone is not flying as fast, actuators and sensors can be the bottleneck. (Note that if we can make an argument for d as well, ie.., depending on d we should also set v, and we should be able to easily get d from piont cloud).  





\subsection{bottleneck and slack relationship}
In this section, we describe the relationship between system's bottlneck and compute slack. Simply put, when not the bottlneck, compute is underutilized. In other words, there is a slack in the time budget for compute to take advantage of. 
\end{comment}


==> tex/dep/impact.tex <==
\section{Potential Long Term Impact} 
\label{sec:impact}
Autonomous mobile machines are on the rise. With myriad use cases in the consumer market (Aerial Photography), industry (Package delivery, Warehouse automation), and government (Search and
Rescue robotics, have more examples), our future societies are painted with men and robots 
coexistence. Although with the advancements made in artificial intelligence and adaptive control, autonomous machines are marching toward reality, plethora of roadblocks stand in the way. These roadblocks stem from the difference between such mobile-cyber-physical (MCP) systems and their traditional counterparts (i.e. desktops, servers, cellphones, etc). We believe that understanding and designing around such difference is the way forward.

The main difference between the mobile-cyber-physical systems and their traditional counterparts is in their mobility, environment interactivity and strict requirements for safety/reliability. These three factors tie physical action very closely to compute. Such a compute/action interdependence imposes a new set constraints on the compute stack traditionally not needed hence not examined extensively. Our tool-set captures compute/action interactions by holistic modeling of the systems environments, sensors, actuators and the compute sub-system.
    
\textbf {Mobility:} Mobility/compute interaction manifests itself in form of the energy and compute resource constraints. Wanting to finish a mission with the limited on board energy requires energy/efficient designs and possibly rethinking the entire compute stack. (some numbers about crazy flie or possibly the drone/car difference would be interesting here). In addition, having to navigate within a host of environments, the machine needs to adapt to absence of certain resources. For example, flying from an outdoor to an indoor environment (street to warehouse), a drone needs to overcome its lack of access to GPS by resorting to more compute intensive localization kernels such as SLAM. Our simulator can capture the aforementioned mobility/compute interactions by faithfully model entire system's (mechanically and electrically induced) energy and environment characteristics. 
    
\textbf{Interactivity:} Constant interaction between the machine and its environment imposes various physical action objectives such as maneuverability, agility, stability, etc. These objectives manifest themselves in form of compute constraints needing to be met. For example, wanting to maintain a collision free mission, MCP machines must process their environment fast enough to react to it. This means, the flow of information depicted in figure blah is strictly bounded by the physical world's requirements.  Our HIL simulator can examine drone's success in achieving the required objectives (e.g. agility) by profiling action metrics (e.g. number of collisions, drone's velocity and acceleration) and compute metrics (e.g. applications latency and throughput). A relationship between compute/interactivity objectives then can be established an example which was provided in the paper. It's also worth noting the unpredictability of the environment (sudden appearance of an obstacle) renders interactivity an even more difficult to problem to deal with. Our simulator can capture such unpredictabilities, for example by modeling dynamic obstacles with random paths. 
     
\textbf{Safety/Reliability:} Having to move within and interact with the environment, system's failure can be catastrophic beyond the machine's own mission failure. A corruption can cause calamitous financial and lethal impacts. Such a problem is then exacerbated given the wider (beyond compute) potential corruption points. As opposed to the traditional systems, MCP systems' compute stack needs to account for sensors' and actuators' corruptions in addition to the compute stack itself. To make things worse, weight, power and energy constraints can limit fault tolerance techniques such as redundancies. Our simulator setup models various noise models for sensors and actuators examples of which was provided in the paper. In addition, weight and energy constraints are captured in our models.
   

    -------------------------------------  

misc: about the need for simulators with the our simulator models energy not only for the compute for the entire system. 
misc: that we mainly focus on motion/compute relationship however, this should be generalized to action/compute.
misc: Maybe talk about cloud/edge connectedness, .
Note: clearning the confusion. Mobile is in contrast with stationary.
overall flow: Maybe first  I can argue about the importance of these systems. 
Then quickly mention that however, these systems are different. Hence new tools are necessary to capture this difference. 
Then I explain how they are different and how our tools capture these differences.



==> tex/dep/long-term-impact.tex <==

%\newpage
%\renewcommand{\baselinestretch}{.2}
\section{Dynamic World, Static Design} 
\label{sec:static_design}
In this section, we highlight the inefficiencies associated with a static design. For both the computational load and the deadline, we show, how a static worse-case design inefficiently uses the compute subsystem. This inturn results in a lower QOF, concretely, the mission time and with it energy. 


\subsection{computation load}
As was mentioned in the previous section, the computational load of navigation pipeline variers throughout the mission as a function of the environment and the sensory subsystem. 
Here we discuss how a static design methodology for space precision and volume, two main performance drivers of spaitial computing, results in an inefficient design. 
\textit{Space precision} The higher the precision, the higher the load and the higher the latency. A static design enforces an immutable static/worse case precision, overly stressing the compute at all times. Figure blah, shows the time sequence associated with a typical flight. Static design, shown in blue, spent an excessive amount of time through out the mission. The difference between the two curves shows the compute inefficiency, where the difference shows the execssive amount of time spent per iteration. On average we see blah sec increase in the time spent on the same amount of space using a static approach. If reduced, this time can be Note that such extra time can bring down the reaction time, improving the velocity and hence the mission time.

\textit{Space volume} The higher the volume, the higher the latency. A static design assumes that the same amount of volume is consumed at any iteration, allocating an extra budget regardless of the actual volume consumed.
Figure blah shows a sequence of volumes consumed by a drone in a a typical flight. The red line shows the staticly allocated budget where as the green line the dynamic counter part. The difference between the two indicates the slack unused. If reduced, this slack can brings down the reaction time, improving the velocity and hence the mission time.

\subsection{computation deadline}
Since the end-to-end deadline is a funciton of the robot speed, such deadline scales wih speed. Figure blah shows sequence of velocity values in a typical flight. The red line shows the static deadline allocated where as the green one the dynamic counterpart. The difference between the two shows the slack unused. If the slack is used, the system can take a higher load when necessary. On average, we see a slack of size blah, with standard devision of blah. 

% The computer architecture community has witnessed major paradigm shifts in computing over the past many decades. We are on the cusp of a new change, as we transition from cloud and mobile computing into an era of autonomous machines. As times changes, so must the systems, tools, and benchmarks that we rely upon to study and unlock new capabilities. 



==> tex/dep/motivation.tex <==
\section{Motivation: MAV cyber-systems need to be co-designed for heterogeneity}

MAVs are cyber-physical systems operating in the real world. As shown in Figure~\ref{fig:heterogeneity}, as they move around their environment, their local physical space varies, changing the inputs sent to and the outputs required from the cyber-system. As such, the cyber-system of an MAV needs to be able to take advantage of this heterogeneity through cyber-physical co-design for optimal performance.

\begin{figure*}[tb!] 
\centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=0.7\linewidth]{figs/space_heterogenity.png}
        \caption{Heterogeneity in space. Three different points along the drone's trajectory are specified (A, B and C). A difference in number and distance to obstacles can be observed for these points.}
        \label{fig:space_res_vis}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=0.6\linewidth]{figs/actuation_heterogeneity.png}
        \caption{Actuation heterogeneity. Three different points along the drone's trajectory(points A, B and C) are specified. The difference in velocity magnitude is denoted by the size of the velocity vector.}
        \label{fig:vel_res_vis}
    \end{subfigure}
\caption{Heterogeneity in a cyber-system's inputs and output requirements.}
\label{fig:heterogeneity}
\end{figure*}

Intuitively speaking, congested areas (i.e., areas with high obstacle counts) demand a high precision understanding of their local environment for safe navigation, requiring high levels of computation. On the other hand, open areas can be traversed quickly with larger, simpler models. At the same time, higher velocity flight leads to shorter time budgets for the cyber-system's computation to ensure that the MAV can stop safely before it runs into a previously unseen obstacle. These changing demands for precision, and changing time budgets afforded to these computations place requirements on the MAV's cyber-system. In order to traverse this space safely, a cyber-system either has to make a worst-case static assumption or be co-designed  on the run time with the physical environment to dynamically adjust to these changing demands.

==> tex/dep/motivation_old.tex <==
%\section{Compute vs. Flight-time vs. Energy Efficiency}
\section{Motivation: cyber-systems need to optimize\\for the physical heterogeneity}

The cyber-system of a MAV needs to be optimized for two main causes of heterogeneity: 1) %is embedded in a heterogeneous framework that is caused by 1. the ever changing
the external/physical world and 2) the internal robot subsystems. Such heterogeneity results in a variation in both the input payload and the output time budgets of the cyber-system. In this section, we quantify these variations, and detail optimization opportunities for a context-aware design.% can take advantage of.
%Since we are targetting navigation and hence spatial-reasoning, we propose "spatial-aware computing" as the corresponding context-aware solution.

%\subsection{Impact of world heterogeneity on the cyber system}
%The ever changing world surrounding the drone imposes a varying demand on the cyber system. Here we quantify such variations and its impact. 

% \todo{Figure part b together --- figure part a is just the visual -- note that the static is an assumed as an example to show concepts -- assumed maximal velocity -- actual and assumed constant maximal or something like that --- make things lines to show that it si maximal and assumed}

% Environment is changing so need to react (congestion level) --- this exists in the real world (disaster response / recovery, agg, indoor -- get some unity environment pics doesn't have to be the actual one used where there is dense vs. light etc). What is the amount of opportunity to go faster? (maybe summarize the results X\% faster) --- this leads to all of these gains (energy, time, success).
% For figure 4b it HAS to be at the bottom and just one line which is "required precision" and if you go static you have to go to the bottom --- and if you move it up you will fail. Then 4b top it will get set all the way at the top. Then to 5 your budget is set so you can only go slow. >>> in a dynamic case you can vary all of these thigns to go faster, use less energy, whatever you want.

\begin{figure*}[tb!] 
\centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/space_heterogenity.png}
        \caption{Heterogeneity in space. Three different points along the drone's trajectory are specified (A, B and C). A difference in number and distance to obstacles (space characteristics) can be observed for these points. Which will vary the inputs to the cyber-system.}
        \label{fig:space_res_vis}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/space_res}
        \caption{Variation of the minimum precision needed for safe navigation (lower graph) impacts the required computational latency (upper graph). A dynamic design adjusts to this variation for higher precision and velocity.}
        \label{fig:space_res_quan}
    \end{subfigure}
\caption{Impact of Variation in the External/Physical World on the Cyber-System} \todo{The color shading is very confusing as the curve colors change I think it should simply be noted to the right of the graph what each section is (@Jon we can talk about this). I also think on the top graph we should only note the Generated time slack section (and therefore use a log plot). On the bottom graph we should call the lower section the "High Precision Sections".}
\label{fig:space_res}
\end{figure*}

\begin{figure*}[t!] 
\centering
   \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=.8\linewidth]{figs/actuation_heterogeneity.png}
        \caption{Actuation heterogeneity. Three different points along the drone's trajectory(points A, B and C) are specified. The difference in velocity magnitude is denoted by the size of the velocity vector.}
        \label{fig:vel_res_vis}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/vel_res}
        \caption{Variation of the velocity during a mission is needed for safe navigation (lower graph) and impacts the time budget available to the cyber-system (upper graph). A dynamic design adjust to this variation allowing it to safely, and efficiently, traverse the entire environment.}
        \label{fig:vel_res_quan}
    \end{subfigure}
\caption{Physical variation impact on the cyber-system output budget.}
\todo{Same note as Figure~\ref{fig:space_res} on coloring. Also I wonder here if we want to say that there is Slack in the velocity in this one as it seems like in the upper chart it is additional required time needed not slack and in the lower the top section is velocity slack that is not taken advantage of?}
\label{fig:vel_res}
\end{figure*}

\textbf{Variation in the External/Physical World:} As the drone moves toward its goal, its surrounding physical space varies changing the inputs sent to the cyber-system. Intuitively speaking, congested areas (i.e., areas with high obstacle counts) demand high precision navigation which imposes a high computational latency. Figure ~\ref{fig:space_res_vis} shows a drone trajectory with 3 way points (A, B and C), each with a different congestion. Point B requires the highest precision due to the high number of close obstacles which in turn demands the highest computational latency. Figure ~\ref{fig:space_res_quan} quantifies the variation in the precision demand and its impact on the response time for an example navigation mission. In this plot, the x axis shows the progression of the mission in seconds, while the y-axis plots the required precision, the lower graph\footnote{Specifically this shows the required minimum voxel side length for safe navigation. Voxels are units of 3D space, an analog to pixels for 2D images.}, and corresponding computational latency, the upper graph\footnote{The response time here indicates how many seconds it takes the cyber-system to compute the required robot commands based on the corresponding voxel side length in the lower graph.}. %The lower graph shows required precision needed for safe navigation, and the y-axis on the upper graph and corresponding response time. We observe an inverse relationship between the precision (bottom  graph, blue curve) and the response time (top graph, blue curve).
% \todo{As seen, a total variation of blah centimeters in precision results in a corresponding response time variation of blah seconds.}

A shown in Figure ~\ref{fig:space_res_quan}, a cyber-system with a constant precision (orange curves) is both incapable of navigating the sections of environment with high precision demands, and cannot take advantage of the time slack generated by the relaxed precision sections. On the other hand, a context-aware dynamic design (blue curves) can can safely navigate all sections of the environment while taking advantage of the time slack to fly faster in non-congested sections or compute additional non-navigation workloads during those times.

\textbf{Variation in the Internal Robot Subsystems:} Along with the external world, variations in internal subsystems (such as actuation) impose a varying time budget on the cyber-system's output. The time budget is defined as the deadline for the cyber-system's computation so that the MAV can stop safely before it runs into a previously unseen obstacle. As such, moments during the flight with high velocity demand a shorter time budget as it takes longer to stop from higher velocities. Figure ~\ref{fig:vel_res_vis} shows a second drone trajectory and 3 points (A, B and C), each with a different velocity. Point B has the highest velocity and thus demands the shortest response time. Figure ~\ref{fig:vel_res_quan} quantifies the variation in velocity and its impact on the time budget for an example navigation mission. 
% We observe an inverse relationship between maximum velocity (bottom graph, blue curve) and time budget (top graph, blue curve). As seen, a total variation of blah m/s in velocity results in a corresponding time budget variation of blah seconds.
A cyber-system that makes static assumptions about the speed at the design time, (orange curves) is both incapable of taking advantage of generated slack in low velocity moments to preform better planning and therefore safely navigate through congested spaces and cannot exceed this static velocity when it is safe to do so. A context-aware dynamic system can, allowing it to safely, and efficiently, traverse the entire environment.

% \begin{comment}

% speaking, as the robot's speed increases, it needs to react to its surroundings faster. This in turn demands faster decision making, and hence lower deadlines per decision. Figure blah depicts this relationship. The data presents the time sequence of a drone's velocity which is tasked with reaching a destination in a collision-free flight. The redline shows how the time budget per iteration varies a function of robot's speed. As seen, we observe a standard deviation of blah x associated with velocity and blahx for deadline.
% Navigation pipeline front end, i.e., environment plus the sensors, determine the computaional load, i.e, the amount of input data to be consumed. Events in the environments are captured through sensors and presented to the cybersystem for interpretation. The richer the environment and the higher the sensory samples, the higher the computational load. 
% Since spatial reasoning sits at the heart of navigation, we consider space as the main processing payload, and further, identify \textit{volume} and \textit{precision} of space as two major drivers of the payload intensity.
% \end{comment}





==> tex/dep/operators.tex <==
\section{Operators}
Operators are responsible for enforcing the policies, i.e., the knob settings decided by the governor. 
As was mentioend previously, we identify space precision and volume as two main payload driver
and thus performance,  consequently, our operators control the these two variables quantity. 
Since the computation associated with spatial reasoning is 
distributed across the perception and planning stages, our operators are spread within each stage, impacting computation, and across them
, impacting communication between them. 
Table blah list all of our operators, their pipeline stage homebase, and a brief description of their impact. 
Although all these operators control seemingly the same variable, i.e., either precision and volume, they semantically
induce different behaviors impact depending on the stage they impact.
\todo{say something about how space volume and precision is the same really, but has 
different impact. Can we find an analogy in the system world}

\subsection{Precision Operators}
There are total of two precision opertors. One controling the precision with which new point cloud is 
integrated into the map, and the other the precision within of the map which the planner explores.
The first one is enabled by controling the sampling rate of the points within the pointcloud.
The second is enabled by taking advantage of the inherent multi-resolution capability of the occupancy map
used.

\subsection{Volume Operators}
There are total of three volume operators, controlling the space volume integrated into the map per iteration,
the potential volume of space that the planner can plan through and finally the accumulated volume of space planner
get to plan through. All of our volume controllers consist of two components, namely a squencer and monitor. 
\subsubsection{Sequencer:} This block is responsible for prioretizing and further orchestrating the order with wich the space will be consumed. 
\subsubsection{Monitor}: This block is responsible for monitoring space volume size. 
The monitor screens the size of the volume that is being released by the sequencer. As the size reaches a threshold
decided by the governor, the monitor signals a termination to the sequencer stoping the consumption of space. 

Here we dicuss the priority policies and their implementation.  \red{I am not sure how to do this.
It just seems like we are too deep in the organizational hierarchy} 


\section{Governor}



\subsection{objective function}

\todo{talk about why the objective function is setup the way it is} 
Equation blah shows the objective function and the constraints. 
The objective function is presented in equation blah, where delta denotes blah ... \red{go over the notation} 
Each one of the delta denote the performance models illustrating the relationship between, space precision, volume and latency.

\todo{talk about how models are collected}Each one of these models are collected through having the drone to fly through various environment.
\subsection{models}


\subsection{constraints}
Equations blah through blah list our equality and inequality constraints. 

\subsection{solver}
We formulate this problem as a optimization problem. 


==> tex/dep/scratch.tex <==
- maybe we can talk about voxel as a unit of work, and hence voxel/sec and voxel/joul
as the compute's figures of merit similar to
MIPS or Instruction per joul.

- note that we gotta be carefull to make sure the paper is not bipolar, torn between spatial computing and dynamicity.

- we might need to mention, why worse-case design is necessary (As opposed to avg case design)


- we should measure the speed of each stage, but calculating teh volume traversed.

- Also we should show how we can track the speed in the dynamic approach.
- can we sell the work as dynamic load controller. Obviously we need tos how how the load is dynamically controlled based on the deadline and the compute capability of the system.

- what if we use xavier and turn off cores (or just not used them) depending on the deadline.


==> tex/dep/slack.tex <==
\section{Slack Deployment}
\label{sec:slack}
In this section, first we discuss how compute not being the bottleneck manifests itself in a slack for the compute stage. Then, we discuss a general approach to take advantage of this slack. Then, we select a host of knobs with which we can improve compute performance and hence reduce the mission time. We take advantage of such knobs when slack is presented to compute. 



\subsection{bottleneck and slack relationship}
In this section, we describe the relationship between system's bottlneck and compute slack. Simply put, when not the bottlneck, compute is underutilized. In other words, there is a slack in the time budget for compute to take advantage of. 

\subsection{compute knobs to exploit the slack with}

==> tex/dep/spatial_computing_old.tex <==
\section{Using Spatial-Aware Computing to Co-Design for Heterogeneity}

This heterogeneity %in both the external/physical world and the internal robot subsystems 
can be capture, analyzed, and optimized for, through our proposed methodology of \textit{spatial-awareness} for cyber-physical co-design.
% spatial reasoning is at the heart of navigation, we propose \textit{spatial-awareness} as the methodology to capture and react to the heterogeneity in space. 
A \textit{spatial-aware} design, continuously captures space characteristics to dynamically adjust the input to and time budgets for the cyber-system. As we will demonstrate later in this work, this improves both mission quality (e.g., mission time) and system efficiency (e.g., utilization). This section introduces \textit{spatial-aware computing} as a cyber-physical co-design paradigm and its fundamental components.

\begin{figure}[t!]
\centering
    \begin{subfigure}{0.44\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/precision_low.png}
   \vspace{-5pt}
   \caption{Low precision implies a low number of large voxels.}
    \label{fig:low_precision}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.44\columnwidth}
    \centering	
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/precision_high.png}
    \vspace{-5pt}
    \caption{High precision implies a high number of small voxels.}
    \label{fig:high_precision}
    \end{subfigure}
  \begin{subfigure}{0.44\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/volume_low.png}
   \vspace{-5pt}
   \caption{Lower volume leads to a lower total number of voxels.}
    \label{fig:low_volume}
    \end{subfigure}
     \hfill
    \begin{subfigure}{0.44\columnwidth}
    \centering	
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/volume_high.png}
    \vspace{-5pt}
    \caption{Higher volume leads to a higher total number of voxels.}
    \label{fig:high_volume}
    \end{subfigure}
\caption{Space precision and volume impact the total number of voxels that need to by processed by the cyber-system.}
\todo{remove borders and play button}
\label{fig:dynamic_precision}
\end{figure}

\begin{figure}[t]
\centering
    \begin{subfigure}{0.49\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/precision_volume_latency.png}
   \vspace{-5pt}
   \caption{Increased space precision and space volume directly increase the computational latency of the MAV's cyber-system.}
    \label{fig:precision_volume_reponse_time_relationship}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\columnwidth}
    \centering	
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/velocity_visibility_budget.png}
    \vspace{-5pt}
    \caption{Increased space traversal speed decreases the computational time budget while increased space visibility allows for an increased budget. Here the mapping stage is used to exemplify these relationship.}
    \label{fig:visibility_velocity_time_budget_relationship}
    \end{subfigure}
\caption{Space precision's, space volume's, space traversal speed's, and space visibility's impact on compute.}
\todo{These graphs are illegible. They need to be simplified, and made larger so they can be understood.}
\label{fig:dynamic_precision}
\end{figure}

\textbf{Spatial Reasoning:} 
\textit{Space} and \textit{spatial reasoning} sit at the heart of navigation. \textit{Spatial reasoning} is the robots ability to reason about its position (absolute or relative) to other objects, to reason about the geometry of such objects, to determine the occupied, free, and unknown space in the environment, and to make optimal decisions about how to traverse the environment. This process requires building \textit{space} related world models and planning actions within them. Each stage in the navigation pipeline is involved in parsing and interpreting space as the main payload, and communication between those stages involves packetizing, serializing, and pushing the encoded space. The amount of space processed by a cyber-system can be controlled through four main variables: \textit{space precision}, \textit{space volume}, \textit{space traversal speed}, and \textit{space visibility}.

\textit{Space Precision:} Space precision, the accuracy with which space is encoded and interpreted by the cyber system, has a direct relationship with the computational latency. Increasing precision, decreases the size of each voxel.\footnote{A voxel is a cube of 3D space, analogous to a pixel in a 2D image.} As a result, a more accurate map uses more, smaller voxels to represent the same space (Figure ~\ref{fig:low_precision} and ~\ref{fig:high_precision}). This leads to a higher latency for each stage of the navigation pipeline as it increases the size of the data that needs to be processed at each stage. As shown in Figure ~\ref{fig:precision_volume_reponse_time_relationship}, doubling the precision will 8x the number of voxels, leading to a \todo{blahx} increase in computational latency.

\textit{Space Volume:} The volume of space processed and interpreted, measured in $m^3$, has a direct relationship with the computational load. The higher the volume, the higher the number of voxels consumed by the pipeline (Figure~\ref{fig:low_volume} and ~\ref{fig:high_volume}). This in turn increases the latency. As shownin Figure~\ref{fig:visibility_velocity_time_budget_relationship}, a 2x increase in volume increases the number of voxels by a factor of \todo{blahx} leading to a \todo{blahx} increase in latency.

\textit{Space Traversal Speed:} The speed with which space is traversed directly impacts the response time budget. Intuitively speaking, the higher the speed associated with the MAV, the smaller the time budget it can have in order to react to and dodge upcoming obstacles. Figure~\ref{fig:visibility_velocity_time_budget_relationship} quantifies this relationship for our MAV showing how increased speed leads to a reduce time budget.  We use a quadratic motion model to generate this graph. The details and methodology for arriving at these models are presented Section~\ref{sec:results}.

\textit{Space Visibility:} The MAV's visibility into the space also impacts the time budget. Intuitively speaking, the further into the space the MAV can see, the further ahead it can observe the obstacles and start planning to avoid them. This in turn gives the drone a higher time budget for response time. Figure ~\ref{fig:visibility_velocity_time_budget_relationship} quantifies this relationship for our MAV which is equipped with 6 cameras showing how increased visibility will also increase the time budget.

\begin{figure*}[!t]
\centering
    \begin{subfigure}{0.66\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/precision_mission_example.pdf}
        \vspace{-5pt}
        \caption{Static (left) vs Dynamic (right) Precision.}
        \label{fig:dyanmic_vs_static_precision}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.66\columnwidth}
        \centering	
        \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/volume_mission_example.pdf}
        \vspace{-5pt}
        \caption{Static (left) vs Dynamic (right) Volume.}
        \label{fig:dynamic_vs_static_volume}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.66\columnwidth}
        \centering	
        \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/response_time_mission_example.pdf}
        \vspace{-5pt}
        \caption{Static (left) vs Dynamic (right) Response Time.}
        \label{fig:dynamic_vs_static_reponse_time}
    \end{subfigure}
    \begin{subfigure}{0.66\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/actuation_velocity_mission_example.pdf}
        \vspace{-5pt}
        \caption{Static (left) vs Dynamic (right) Traversal Speed}
        \label{fig:dynamic_vs_static_velocity}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.66\columnwidth}
        \centering	
        \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/sensor_visbility_mission_example.pdf}
        \vspace{-5pt}
        \caption{Static (left) vs Dynamic (right) Visibility}
        \label{fig:dynamic_vs_static_visibility}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.66\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\columnwidth]{figs/time_budget_mission_exmple.pdf}
        \vspace{-5pt}
        \caption{Static (left) vs Dynamic (right) Time Budget}
        \label{fig:dynamic_vs_static_time_budget}
    \end{subfigure}
\caption{Space Precision, Volume, Response Time, Traversal Speed, Visibility, and Time Budget for static and dynamic cyber-systems for a sample trajectory through an environment.}
\todo{Drop the numbers from both axis they are irrelevant. Also the way the scales are now it looks like the static and dynamic are the same response time at the end. Might want to use a log scale. We don't reference Point A in d,e,f so remove it.}
\label{fig:Spatial_aware_design}
\end{figure*}

\textbf{Using Spatial-awareness to Enable Cyber-Physical Co-Design:} A \textit{spatial-aware} design, continuously captures space characteristics to dynamically adjust these variables. On the other hand, a \textit{spatially-oblivious} design, sets such variables statically at design time, and maintains them through out the mission. This requires both setting these variables for worse-case scenarios and continuously re-tuning them for each specific mission. Figure~\ref{fig:Spatial_aware_design} compares a \textit{spatial-aware} vs \textit{spatial-oblivious} design for an example navigation mission. Each figure shows a top-down view of the environment with the black squares signifying the position of obstacles. The heatmap shows the variable of interest as the MAV navigates around these obstacles. In each figure the left graph shows the static, \textit{spatially-oblivious} design, while the right graph shows the dynamic, \textit{spatial-aware} design.
% The reader can trace drone trajectory by following the arrows along of colored squares. 
% As we will detail later, the former excessively pressures the compute with unnecessary computations and the latter degrades the adaptability and scalability of the cyber-system to new mission types.

As seen in  Figure ~\ref{fig:dyanmic_vs_static_precision} and ~\ref{fig:dynamic_vs_static_volume}, the \textit{spatially-oblivious} design uses a constant precision and volume where as the \textit{spatial-aware} design dynamically adjusts them. For example, as the MAV gets closer to obstacles it increases its precision. This can be seen near Point A in Figure~\ref{fig:dyanmic_vs_static_precision} as the heatmap transitions from green to yellow as the MAV nears the obstacle. Figure~\ref{fig:dynamic_vs_static_reponse_time} shows the response time impact of such design decisions. The static design always spends the same amount of computation regardless of the space demands which in turn excessively over utilizes the compute and doesn't allow for faster flights. On the other hand, a \textit{spatial-aware} design optimizes its desired response time, allowing for additional compute in uncongested areas. We quantify this impact in detail in Section~\ref{sec:results}.

Figure ~\ref{fig:dynamic_vs_static_visibility} and ~\ref{fig:dynamic_vs_static_velocity}, show that the \textit{spatially-oblivious} design also makes a static assumption about its velocity and visibility in order to ensure worst case safe flight. The dynamic design, on the other hand, can optimize its settings to the environment. Figure~\ref{fig:dynamic_vs_static_time_budget} shows the time budget impact of such design decisions. The static, \textit{spatially-oblivious} design always assumes a small time budget where as the \textit{spatial-aware} counter part increases its response time, flying faster, with farther visibility in uncongested areas.
% The slack associated with the extra time budget can also be used by dynamic design for other non-navigation tasks. 
We quantify these benefits in detail in Section~\ref{sec:results}.


% \begin{comment}
%  A static design enforces an immutable static/worse case precision at all time because it is incapable of adapting to the changes in precision
%  requirements. \todo{can we elaborate a bit more} 
% Figure blah illustrates this by presenting the required, and the corresponding statically and dynamically imposed precisions. Concretely, the curve in purple presents the time
% sequence of a required precision associated with a flight \footnote{we use gaps as a proxy for precision requirements}. As seen, precision varies drastically throughout by as much as blah percent
% (for worse case difference) and with standard deviation of blah. The curve in red shows the imposed static precision with an tracking error avg of blah and std of blah.\footnote{tracking error is defined as blah}.
% In contrast the green curve shows our dynamicly imposed precision which reduces the tracking error to blah percent. 

% Static/worse-case design overly pressures the compute at all times regardless of the space precision requirements. Figure blah presents the latency corresponding static (red line) and dynamic (green
% line)
% design. The difference between the two curve shows the magnitude of the inefficiency, i.e, the excessive time spent on space. A static design incures an execcsive latency of up to blah (for worse
% case) and average of blah. Note that the dynamic design's reduced latency brings down the reaction time, and hece improving velocity and mission time. This imapct is detailed thoroughly in chapter blah.






% Space Volume  dynamically changes based on environmental factors such as occlusion. Intuitively speaking, a robot whose vision is considerably blocked from different directions consumes less volume than a robot surrounded by free space. Figure blah depicts the dynamic nature of volume. As our drone traverse an area, it is occluded at different times with different intensity and so does with it the payload. As seen, for this flight, we observe a standard deviation of blah for the volume.



% \todo{Say something about this paper making at attempt at this domain. I don't know is what are  the components that we need to cover to lift a field off the ground. Possibly we can mention how
% each section discuss different components. Also should we have a paragraph discussing 
% the relevance of each section to spatial computing components.}
% The studies presented in this paper examplify the type of problems, methodologies, and metrics
% that the designers of this domain deal with.  








% A static design assumes consumption of a fixed/worse-case space volume at all times since it is incapable of tracking volume changes. 
% Figure blah illustrates this by presenting the actual volume consumption, and the corresponding dynamic and static tracking of it. Concretely, the curve in purple presents the time sequence of the
% actual volumes consumed through out a flight. As seen, volume varies drastically throughout by as much as blah percent
% (for worse case difference) and with standard deviation of blah. The curve in red shows the assumed static volume, with an tracking error avg of blah and std of blah.
% In contrast the green curve shows our dynamicly tracking of the volume which reduces the tracking error to blah percent. 

% Static/worse-case design allocates a fix time budget at all times to process space volume. 
% Figure blah presents the budget corresponding to static (red line) and dynamic (green
% line)
% design. The difference between the two curve shows the magnitude of the inefficiency, i.e, the excessive time budget allocatedfor space processing. A static design overbudgets the system by as much as  blah (for worse
% case) and average of blah. 

% The excessive budget either under or over utilize the compute. \footnote{something about redundanc}. By adjusting the budget,
% the dynamic design brings down the reaction time, and hece improving velocity and mission time. This imapct is detailed thoroughly in chapter blah.


% \textbf{ Dynamic Deadline (budget)} Navigation pipeline backend, i.e., the environment and the acutation determine the compute deadline. Intuitively speaking, as the robot's speed increases, it needs to react to its surroundings faster. This in turn demands faster decision making, and hence lower deadlines per decision. Figure blah depicts this relationship. The data presents the time sequence of a drone's velocity which is tasked with reaching a destination in a collision-free flight. The redline shows how the time budget per iteration varies a function of robot's speed. As seen, we observe a standard deviation of blah x associated with velocity and blahx for deadline. 

%  A static design assumes worse-case velocity at all times since it is does not track veloity changes. 
% Figure blah illustrates this by presenting the actual velocity, and the corresponding dynamic and static tracking of it. Concretely, the curve in purple presents the time sequence of the
% actual velocity through out a flight. As seen, velocity varies drastically throughout by as much as blah percent
% (for worse case difference) and with standard deviation of blah. The curve in red shows the assumed static velocity, with an tracking error avg of blah and std of blah.
% In contrast the green curve shows our dynamicly tracking of the velocity which reduces the tracking error to blah percent. 

% Static/worse-case design allocates a fix time budget at all times to react to the assumed "fixed" velocity. 
% Figure blah presents the budget corresponding to static (red line) and dynamic (green
% line)
% design. The difference between the two curve shows the magnitude of the inefficiency, i.e, the excessive time budget allocated. A static design overbudgets the system by as much as  blah (for worse
% case) and average of blah. The excessive budget  can be used to consume more payload to improves optimality of robots decision making.
% \end{comment}


==> tex/dep/static_design.tex <==
\subsection{Motivation: Dynamic world yet static design}
\label{sec:static_design}
 %A static design enforces an immutable load (associated with the worse case gap size) overstressing the compute at all times. The difference between the optimal load and worse case load has an impact on the end-to-end response time as shown in figure blah. 
%A static design assumes an immutable volume (load) throughout the mission allocating time appropriate for a worse case scenario volume. Figure blah shows the slack associated with the latency of worsecase volume and the changing volume throughout a flight. 
%A static design enforces a immutable deadline for a worsecase velocity as shown. As seen, this approach would ignore the budgetheadroom shown inducing a time slack unused. 

\label{sec:static_design}

\if\briefmode1
\begin{briefenv}
\brief{Detail static design inefficiencies by describing and quantifying shortcomings ass/w static assumptions. }

- Static paypload (quantify tracking error and impact). 

\hspace{3ex} - Static precision.

\hspace{3ex}
-  Static volume.

- Static deadline(quantify tracking error and impact).
\end{briefenv}
\else
In this section, we highlight the inefficiencies associated with a static design which targets aforementioned dynamic system. Concretely, we show how a static worse-case design inefficiently uses the compute subsystem by ignoring the dynamicity within both the computational load and the deadline. This inturn results in a lower \textit{quality of motion} metrics such as mission time and with it energy. 


\subsubsection{Static Computational Payload}
The computational payload varies throughout the mission.
Here we discuss how a static design methodology for space precision and volume, two main payload drivers of spaitial computing performance, results in an inefficient design. 

\textbf{Static Space Precision}
 A static design enforces an immutable static/worse case precision at all time because it is incapable of adapting to the changes in precision
 requirements. \todo{can we elaborate a bit more} 
Figure blah illustrates this by presenting the required, and the corresponding statically and dynamically imposed precisions. Concretely, the curve in purple presents the time
sequence of a required precision associated with a flight \footnote{we use gaps as a proxy for precision requirements}. As seen, precision varies drastically throughout by as much as blah percent
(for worse case difference) and with standard deviation of blah. The curve in red shows the imposed static precision with an tracking error avg of blah and std of blah.\footnote{tracking error is defined as blah}.
In contrast the green curve shows our dynamicly imposed precision which reduces the tracking error to blah percent. 

Static/worse-case design overly pressures the compute at all times regardless of the space precision requirements. Figure blah presents the latency corresponding static (red line) and dynamic (green
line)
design. The difference between the two curve shows the magnitude of the inefficiency, i.e, the excessive time spent on space. A static design incures an execcsive latency of up to blah (for worse
case) and average of blah. Note that the dynamic design's reduced latency brings down the reaction time, and hece improving velocity and mission time. This imapct is detailed thoroughly in chapter blah.

\textbf{Static Space Volume} A static design assumes consumption of a fixed/worse-case space volume at all times since it is incapable of tracking volume changes. 
Figure blah illustrates this by presenting the actual volume consumption, and the corresponding dynamic and static tracking of it. Concretely, the curve in purple presents the time sequence of the
actual volumes consumed through out a flight. As seen, volume varies drastically throughout by as much as blah percent
(for worse case difference) and with standard deviation of blah. The curve in red shows the assumed static volume, with an tracking error avg of blah and std of blah.
In contrast the green curve shows our dynamicly tracking of the volume which reduces the tracking error to blah percent. 

Static/worse-case design allocates a fix time budget at all times to process space volume. 
Figure blah presents the budget corresponding to static (red line) and dynamic (green
line)
design. The difference between the two curve shows the magnitude of the inefficiency, i.e, the excessive time budget allocatedfor space processing. A static design overbudgets the system by as much as  blah (for worse
case) and average of blah. 

The excessive budget either under or over utilize the compute. \footnote{something about redundanc}. By adjusting the budget,
the dynamic design brings down the reaction time, and hece improving velocity and mission time. This imapct is detailed thoroughly in chapter blah.

\subsubsection{Static Computational Deadline}
 A static design assumes worse-case velocity at all times since it is does not track veloity changes. 
Figure blah illustrates this by presenting the actual velocity, and the corresponding dynamic and static tracking of it. Concretely, the curve in purple presents the time sequence of the
actual velocity through out a flight. As seen, velocity varies drastically throughout by as much as blah percent
(for worse case difference) and with standard deviation of blah. The curve in red shows the assumed static velocity, with an tracking error avg of blah and std of blah.
In contrast the green curve shows our dynamicly tracking of the velocity which reduces the tracking error to blah percent. 

Static/worse-case design allocates a fix time budget at all times to react to the assumed "fixed" velocity. 
Figure blah presents the budget corresponding to static (red line) and dynamic (green
line)
design. The difference between the two curve shows the magnitude of the inefficiency, i.e, the excessive time budget allocated. A static design overbudgets the system by as much as  blah (for worse
case) and average of blah. The excessive budget  can be used to consume more payload to improves optimality of robots decision making.



\fi

% The computer architecture community has witnessed major paradigm shifts in computing over the past many decades. We are on the cusp of a new change, as we transition from cloud and mobile computing into an era of autonomous machines. As times changes, so must the systems, tools, and benchmarks that we rely upon to study and unlock new capabilities. 




==> tex/introductions.tex <==
\section{Introduction}
\label{sec:introduction} 

In short we make the following contribution:
\begin{itemize}
    \item  We provide the first Gable based simulator combining the agility of gable's analytical models and the fidelity of event driven simulators.
    \item  We provide a design space exploration framework for accelerator rich SoCs. The complexity of these systems resulting in an enormous design space size demands agile DSEs. We formulate our exploration heuristic with simulated annealing focused on bottleneck reduction (building on top Gables strengths). 
    DSE's proposed in literature either target multicore design, microarchitecture parameter tunning, use genetic algorithms or only target allocation or mapping problem. In contrast we use a simulated annealing for accelerator rich SoCs solving the mapping and partitinoing problem simaltenously.
    \item As FARSI is deployed in the initial design stages, it uses agile yet low fidelity IP models as input. We provide sensitivity analysis quantifying the impact of input error on the output fidelity and development cost. 
    We augment our heuristic to dampen this impact by considering the error distribution. 
    \item  As the PPA constraints of the aforementioned SoCs results in great deal of customization and thus development cost, we build cost-awareness into the DSE. As we will show, our heuristic both intrinsically as it traverses the space, and explicitly (through scheduling cost reduction passes) minimizes the development cost. 
   
    \item we characterize ILLIXR workload.
\end{itemize}



What's the work about:
    Random thoughts: what if we sell this as a platform, similar to llvm, and implement a couple of solutions proposed in micro in the system and show that 1. we can replicate other research 2. people can try out their ideas on it. Basically the idea is to sell this as a llvm for system level estimation enabling, topology generation (interconnect research), datamovement (locality research), memory parallelism and placement,  scheduling, mapping (run time research),  ??. Discuss modularity of moves (and how we can think of them as passes). Also, discuss, we can run machine learning on it. 

    what's missing as a toolset is a augmentable DSE (similar to llvm). Both the overall heuristic and the moves (passes) can be augmented in FARSI. 

    The argument here is that designing accelerators individually is not good enough, rather a system level analysis to determine the perforance/power budget per acceleartor is necessary. This is important as the customization (time spent on each kernel) is pretty important in accelerator rich systems, hence a framework that identify the metric targets, is necessary. 


    we can also sell the work as determining the system specs (determing how much speed up do you neeed to get from each acceleartor. Look into this from gabels).


Simulation/Modeling
Cycle accurate vs analytical (trading off performance vs accruacy). we acommpish both. Others are trace-based trying to capture the behavior on one platform and map the computation to another device. These work generally at the instruction level and generally slow. 
Simulators dveloped for specfic systems (Cpu, GPU) or NoCs we raise the abstraction level to the system and provide a general model for the system. 


DSE:
Related work either focuses on binding or allocation,
or uses genetic alogrithms.
Also some of the approaches target MPSOC and not acceleartor rich systems.j
A considerable number of work target resource management of existing systems (i.e., given  a system, how to improve its effcieiy through improving utilization, ...). These work ar orth0ogonal to our work as we target system assmebly/generation. 


Custom SOC
    Accelerator design:
        Other works have been proposed to improve/acclerate/alleivate the accelerator design/methodology. These works are orthogolonal to our work. 
    System Design:
        reconfigurable design stuff.
        
        
        
Given the complexity of today's systems, we advocate higher level system models with enough accuracy and design exploration at the level system. works like gem5-aladdin and gem5-salam attamps at taking a holistic look at the system level, however, they still consier cycle accuracy and result in low simulation perforamnce for accelerator rich systems with 40-50 accelerators.


Multiple frameworks (alaadin, accelSeeker, Execution Time Prediction for Energy-Efficient Hardware Accelerators
Tao) have proposed accelerator simulation/modeling to capture the acceleartor performance/power, ... in isolation. Our work is orthogonal to these works as we raise the abstraction to system level and hollistically model the wholse systems. In this work, we use acccelSeeker. 

Various languages are propose to imporove/accelerate the accelerator design. (refer to A Compiler Infrastructure for Accelerator Generators
Extended Abstract  paper). These papers are orthogonal to our work as they can help improving/acclerator the system design process after the system is estimated.

Posisbly we can discuss work that provide reconfigurable platforms or work on developing a methodlogy to provide an efficient reconfiguratble platforms.


Previous work in the arthicteure community has focuesed on desktop/server/mobile workloads systems of which are not under as much tight constrained or mainly IMAGE processing kernels (JPEG, H264) workloads in the embedded system community. In this work, we provide insights into the AR/VR benchmarks as we believe, the system containing these workloads have the characteristics necessary for accelerator rich systems. In this work, we shed light on various benchmarks within this domain by analyzing and providing systems for them. 

I wonder if I can make claims such as the way that platform is defined, new moves (regarding mapping, allocation, binding, ...) can be easily added. 


As the tool is used at the inital stages, it does have to take into account the error models of the input. 


some methodologies, do the work in mulitple steps, like topology generation (some heursitc), then do allocation and bonding (possible genetic algorithms), some do computational first then do commuinncatino. We do all at the same time. 


we might be able to argue that all the other DSE's formulations do not take advantage of the architects knowledge, as they are simply formulated blindly. However, our augmentable approach, allows for designers knowledge to be integrated into the DSE. 
%We augment our simulator with a simulated annealing heuristic providing an agile an automated DSE framework necessary for the accelerator rich SoCs of the future. 


==> tex/mav_complex.tex <==
\subsection{Hardware Layer}
\label{sec:MAV_subsystems}
\if\briefmode1
    \begin{briefenv}
    \brief{MAV system complex components and interactions.}
    \end{briefenv}
\else
\begin{comment}
\begin{figure}[t!]
\centering
\includegraphics[trim=0 0 0 -25, clip, width=.6\linewidth]{figs/drone_components.pdf}
\caption{MAV robot complex. The three main subsystems, i.e., compute, sensors and actuators, of an off-the-shelf Intel Aero MAV are shown. All other MAVs have a similar subsystem structure.}
\label{fig:drone_components}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[t!]
\centering
    \begin{subfigure}{0.44\columnwidth}
    \centering
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/drone_components.pdf}
   \vspace{-5pt}
   \caption{Robot complex.}
    \label{fig:low_precision}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.44\columnwidth}
    \centering	
    \includegraphics[trim=0 0 0 0, clip, width=0.9\columnwidth]{figs/feedback.png}
    \vspace{-5pt}
    \caption{world=robot feed back.}
    \label{fig:high_precision}
    \end{subfigure}
\caption{Robot complex/environment interaction.}
\label{fig:dynamic_precision}
\end{figure}

\end{comment}


\begin{figure*}[!t]
\centering
\includegraphics[trim=0 0 0 0, clip, width=.9\linewidth]{figs/runtime_arch_flow/roborun_overall_arch_v8.png}
%\includegraphics[trim=0 0 0 -25, clip, width=\linewidth]{figs/navigation_pipeline.png}
\caption{Our navigation pipeline (pink) augmented with our runtime middleware (green). Thicker arrows show the full pipeline task flow, and thinner ones show the dataflow in/out of runtime.}
\label{fig:PPC_pipeline}
\end{figure*}

Robots have three main subsystems: sensing, actuation, and compute (Figure~\ref{fig:PPC_pipeline}, bottom layer). Data flows in a closed-loop from the environment to the MAV's sensors, compute, and actuators, sequentially, and then back to the environment.
%Similar to other cyber-physical systems, the design and development of MAVs requires an understanding of their composed and intertwined subsystems which we detail in this section. 
\textit{Sensors} capture the robot's state and its surrounding environment. 
Robots must be equipped with a rich set of sensors such as \mbox{RGB-D} cameras, to enable intelligent flights. 
%to determine obstacle distances and positions. 
Sensory data are provided to compute.
%The number and the type of sensors are highly dependent on the workload requirements.
The \textit{Compute subsystem} is comprised of two components, a companion computer responsible for computationally intensive tasks (e.g., computer vision) and a motor controller responsible for conversion from high to low-level actuation commands. Compute commands are sent to 
\textit{Actuators} that allow the robot to react to its surroundings. %ranging from rotors to robotic arms.  

We use Micro Aerial Vehicles (MAV) as the example robot platform due to their multiple use cases. We use a quadrotor MAV with six camera sensors providing a near 360-degree field of vision, an inertial measurement unit (IMU), a GPS sensor, and a companion computer for the application layer.

%\textbf{Flight Controller (Compute):} The flight controller (FC) is an autopilot system responsible for the MAV's stabilization and conversion of high-level to low-level actuation commands. 
%While they themselves come with basic sensors, such as gyroscopes and accelerometers, they are also used as a hub for incoming data from other sensors such as GPS and sonar. For command conversions, FCs take high-level flight commands such as``take-off" and lower them to a series of instructions understandable by actuators (e.g., current commands to electric motors powering the rotors). FCs use light-weight processors such as the ARM Cortex-M3 32-bit RISC core for the aforementioned tasks.    
 

%Not all MAVs come equipped with companion computers. Rather, these are typically an add-on option for more processing. NVIDIA's TX2 is a representative example with significantly more compute capability than a standard FC.


\fi


==> tex/results.tex <==
\section{Results} \label{sec:results}

In this section, we first present our overall results and then
evaluate our design's sensitivity to environment difficulty/heterogeneity. Finally, we provide a low-level analysis through the lens of a representative mission.

To evaluate RoboRun robustly, we use our environment generator to vary space difficulty/heterogeneity by varying obstacle density, spread, and goal distance (Table~\ref{fig:eval_scenarios}). We use 3 values for each, resulting in 27 test environments. Each run emulates a package delivery or search and rescue mission with two congested zones at the beginning and end (emulating two warehouses or hospital/building combinations) and a middle non-congested zone (emulating open skies/over the city). 

\begin{table}[t]
\centering
\small
\begin{tabular}{|c|c|}
\hline
\textbf{Environment Knobs} & \textbf{Dynamic Values} \\ \hline
Obstacle Density            & {[}0.3, 0.45, 0.6{]}    \\ \hline
Obstacle Spread          & {[}40, 80, 120{]}       \\ \hline
Goal Distance              & {[}600, 900, 1200{]}    \\ \hline
\end{tabular}
\caption{Evaluation scenarios.}
\label{fig:eval_scenarios}
\end{table}


%Finally, we expand our data-set measuring 

%over high level mission metrics such as mission time and energy and their corresponding improvement. Then, we detail the impact of compute on these metrics, specifically connecting the cyber metrics such as latency/throughput to the over all mission time.
%possibly show slack.

%\subsection{Mission Metrics}
%Show the improvement on QOF accross environements. 
%Then discuss how mission time depends on distance travelled and velocity (d/v).



\subsection{Mission Time, Energy and Velocity Improvements}
We compare RoboRun against a baseline spatial oblivious design using overall mission time and mission energy as our overarching metrics. %. We focus on mission time and energy as two main QoS metrics since improving the former, for example cutting it in half, potentially doubles the delivered packages or victims found, and improving the latter enables more/longer missions. 
The results are collected and averaged over all difficulty levels for all environments (see Figure~\ref{fig:mission_metrics}).


\begin{figure}[h]
\centering
%\includegraphics[width=0.84\columnwidth]{figs/overall_summary_metrics.png}
\includegraphics[width=0.9\columnwidth]{figs/overall_summary_metrics_alt.png}
%\vspace{-0.5em}
\caption{Mission level metrics for two designs.}
\label{fig:mission_metrics}
\end{figure}


% mentioned above to show the overall improvements regardless of the environment difficulty level. 
% \textbf{Flight Time:} 
% We find that our spatial-aware design reduces the flight time by 5X. 

\textbf{Flight Velocity.} By adjusting precision and volume knobs continuously, RoboRun improves velocity by 5X (from 0.4~m/s to 2.5~m/s). By lowering the precision and volume when possible, RoboRun reduces each decision's latency, improving the drone's reaction time, enabling a faster collision-free flight.
%improving the drone's reaction time to doge obstacles and hence enables a faster collision free velocity.
%which can then meet the short deadlines associated with higher velocities. 

%This in turn enables agile flights and lowers the overall mission time by as much as 4.5X (from 2093~(s) to 465~(s)). 

\textbf{Flight Time.} RoboRun's higher velocity enables a faster package delivery or search and rescue mission. The aforementioned 5X improvement in velocity allows the drone to traverse the space faster and arrive at its destination more quickly. RoboRun improves the overall mission time by as much as 4.5X (from 2093~(s) to 465~(s)). 

%taking advantage of lower conge latency associated with low congestion areas,   allowing for faster flight resulting in a 5X reduction in flight time.
% \textbf{Flight Energy:}

\textbf{Flight Energy.} RoboRun also improves energy consumption by 4X (from 1000~kJ to 257~kJ). This improvement occurs because flight energy is highly correlated with flight time, as propellers consume large amounts of energy even when hovering, i.e. zero velocity \cite{boroujerdian2018mavbench}. Therefore, lowering flight time reduces energy usage. Note that since compute consumes less than 0.05\% of the overall MAV's energy \cite{boroujerdian2018mavbench}, reducing compute energy consumption does not directly impact the overall mission's energy. Instead, compute's impact is through increasing velocity, reducing flight time, and hence, flight energy.

\textbf{System Utilization.} As shown in Figure~\ref{fig:mission_metrics}, RoboRun reduces CPU-utilization by 36\% on average per decision as it lowers the computational load when the environment allows it. This in turn frees up CPU resources for higher-level cognitive tasks such semantic labeling \cite{redmon2016you}, image segmentation \cite{nguyen2019mavnet}, gesture \cite{kopuklu2019real}, action detection \cite{duarte2018videocapsulenet}, warehouse \cite{eudes2018autonomous} and infrastructure inspection \cite{sa2017weednet}. Since navigation is a primitive workload, lowering its pressure on CPU is imperative.
%so that higher-level cognitive tasks such semantic labeling \cite{redmon2016you}, image segmentation \cite{nguyen2019mavnet}, gesture \cite{kopuklu2019real} and action detection \cite{duarte2018videocapsulenet}, warehouse \cite{eudes2018autonomous} and infrastructure inspection \cite{sa2017weednet} are enabled. 
%crop health evaluation \cite{sa2017weednet} are enabled.
%then  to be used by non-navigation, yet critical tasks such as \textit{semantic labeling}.  This is important as navigation is primitive and hence lowering the utilization ....  


\subsection{Robustness Across Environment Heterogeneity}

We explore RoboRun's sensitivity to the environment with different difficulty levels. We show that regardless of environment difficulty, RoboRun performs significantly better than a baseline oblivious to an environment's spatial heterogeneity. 

As mentioned earlier, we control environment difficulty by varying obstacle density, spread, and goal distance (Table~\ref{fig:eval_scenarios}). Each randomly generated environment contains two congested (A and C) zones and one non-congested (B) zone. Congested zones are located at the beginning and end of the mission to emulate warehouse-building or hospital-building combinations. These zones are heterogeneous, with a gradual reduction of congestion outward from their center. In contrast, zone B is homogeneous and bigger, representing a longer distance traveled, either in open skies or over a city. Figure \ref{fig:env_sensitivity} shows the sensitivity results and ~\ref{figs:congestion_map} shows a sample mission.

% how environments with varying difficulty degrees impact the two designs. 
% Difficulty is imposed across three knobs, i.e., congestion peak, congestion spread and goal distance. Each knob are swept for 3 different values (table blah \red{jon} \red{behzad}) amounting to 27 type of environments each with a different difficulty degree. 8 experiments are ran per environment difficulty with position of the obstacles randomized for every run. The environments have two centroids (similar to figure ~\ref{figs:congestion_map}) with zones A/C congestion imposed according to the difficulty level. Zone B is homogeneously free.

%impact of each pipline stage on response time.  (This is a good place to discuss sensitivity). Specifically show how sensitivity changes depending on the space requirements. Also discuss the control flow paths (assensment and planning) and discuss how often each path is 
%taken (this impacts the time spent on each stage)


%\subsection{Evaluation Scenarios:}


\textbf{Obstacle Density:}
The peak density and spread of obstacles impact the space difficulty by affecting the obstacle count and their relative distance from each other. A higher obstacle density negatively impacts mission time and energy (Figure~\ref{fig:env_sensitivity}, top left) by resulting in more closely placed obstacles, demanding a higher precision, higher latency computation, and, hence, a lower affordable velocity. RoboRun and the baseline experience a worst-case 1.5X and 1.1X increase in flight time (from 390~(s) to 574~(s), and 1978~(s) to 2244~(s)), respectively, across the highest and lowest density environments. RoboRun is more sensitive to the environment difficulty as it exploits easier environments whereas the poorer performance of the baseline is less impacted.
%We note that this knobs negative impact on velocity is the cause of flight time slow down. As shown, this is reflected in the spatial-aware design again being effected more than the spatial-oblivious design. (1.3X vs no impact). 
Energy closely follows flight time. 


\textbf{Obstacle Spread:} It determines the obstacle distribution across an environment. RoboRun and the baseline experience an increase in flight time by as much as 1.4X and 1.1X (from 383~(s) to 556~(s), and 1996~(s) to 2228~(s)), respectively, across the highest and lowest spread environments (Figure~\ref{fig:env_sensitivity}, top right). %, and a velocity slow down of 1.4X and none, 
Note that spread has a smaller impact on the designs as it mainly determines the area over which obstacles are distributed as opposed to their density. 

\begin{comment}
Figure ~\ref{fig:congestion_sensitivity_analysis_heat_map} shows the compounding impact of the obstacle density and spread on mission time metrics with X and Y axis denoting obstacle spread and density respectively. The heat-map shows the relative flight-time variation normalized to the easiest setup (density = .3 and spread = 40). The severity of environment impact on mission time can be observed with severity of color changes within the map. As expected, RoboRun design's colors change more drastically.
For this design, fixing the spread at 40m (first column), we can see a 50\% increase in mission time as we increase the peak density from the easiest (0.3) to hardest (0.6) environment. On the other hand, similarly fixing the spread at 120m results in a 65\% increase in mission time. Intuitively speaking, this means that the impact of obstacle spread is more severe for higher peak density and vice versa. This indicates that the compounding impact of obstacle peak density and spread can not be simply reduced to a linear relationship.
\end{comment}

\begin{figure}[t]
%\includegraphics[width=\columnwidth]{figs/flight_time_varying_params.png}
 \hspace*{-1.1em}
\includegraphics[trim=3 0 7 0, clip, width=1.05\columnwidth]{figs/flight_time_varying_params.png}
%\vspace{-1.5em}
\caption{Sensitivity analysis across different difficulty knobs.}
\label{fig:env_sensitivity}
\end{figure}



\textbf{Goal Distance:}
As goal distance increases, so does mission time. Goal distance increases flight time for RoboRun and the baseline by as much and 1.3X and 2X (from 399~(s) to 514~(s), and 1482~(s) to 2955~(s)), respectively (Figure~\ref{fig:env_sensitivity}, bottom). RoboRun can minimize the impact of the increased goal distance by swiftly flying through non-congested areas. However, the baseline is heavily impacted by the goal distance due to its constant velocity, making long-distance flights necessary for package delivery and search and rescue, often infeasible for the baseline as longer flight times expend the battery.


\subsection{Representative Mission Analysis}


\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{figs/map_congestion_trajectory.png}
%\vspace{-.75em}
\caption{The heat map signifies each points' congestion level. X and Y axis are Cartesian space coordinates of the space traveled. Our missions contain 3 zones. Zone B is bigger and less congested emulating open-skies/over city and Zone's A/C are smaller/more congested emulating a congested warehouse/hospital/building at the beginning and end of a package delivery/search and rescue mission.}
\label{figs:congestion_map}
\end{figure}


To better understand how RoboRun arrives at the previously discussed improvements, we analyze a representative mission in detail. Our mission takes place in an environment with the mid-range difficulty level (as shown in Figure~\ref{figs:congestion_map}) %concretely congestion peak = 0.45, congestion spread = 120 (m) and  goal distance = 900,  
to avoid skewing the result toward either extreme of environment difficulty. As mentioned before, the trajectories across two runs (even of the same design) vary due to the planner's stochastic nature. Nevertheless, the trends are worth analyzing.  
%In this section, we detail how spatial-aware computing impacts flight time and energy (physical metrics). Concretely, we show how computation/communication (cyber metrics) are adjusted to respond to space heterogeneity drivers, precision and volume, ultimately improving the mission. We compare our spatial-aware to an spatial-oblivious design for a representative environment.
%The results are provided the decision granularity so the reader can observe a finer understanding the design.
%Our mission takes place in an environment within the mid-range  difficulty level (Figure ~\ref{figs:congestion_map}, concretely congestion peak = 0.45, congestion spread = 120 (m) and  goal distance = 900,  to avoid skewing the result toward either end of environment difficulty spectrum.  The path taken by the spatial aware/oblivious designs are shown with arrows in the left and right graph respectively. As we mentioned before, the trajectories across two runs (of even the same design) vary due to the stochastic nature of planner. Nevertheless, the trends are worth analysis. 



% \begin{figure}[t!] 
%     \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/knob_setting_values.png}
%         \label{fig:knob_setting_values}
% \caption{Knob setting value(s) for the dynamic and static designs. Spatial-oblivious design only uses one value determined at the design time, where as the spatial-aware design uses the knob range to react according to its environment.}
% \label{fig:res_quan}
% \end{figure}


\textbf{Mission Metrics:}
RoboRun improves mission time and energy usage by around 3.5X and 3X (from 2096~(s) to 600~(s), and 961~kJ to 331~kJ), respectively (Figure~\ref{fig:sample_flight_time_energy}). Note that RoboRun spends a short amount of time in zone B compared to the baseline as it can take advantage of this zone's low congestion. As mission time ($t$) is determined by the distance traveled ($d$) and average velocity ($v$), i.e. $t = d/v$,
% $Mission\;Time = d/v$ describes the variables impacting mission time with $d$ and $v$ denoting distance travelled and average velocity. 
here we discuss each variable in detail. 

% \begin{equation}
%      \label{eq:mission_time}
%      \text{Mission Time } = \frac{d}{\bar{v}}.
% \end{equation}

\begin{figure}[t]
\centering
    \begin{subfigure}{\columnwidth}
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/sample_mission_flight_time_energy_legend.png}
        %\vspace{-1.8em}
    \end{subfigure}
    
    \begin{subfigure}{0.6\columnwidth}
        \includegraphics[valign=t, trim=0 0 0 0, clip, width=\linewidth]{figs/sample_mission_flight_time_energy.png}
    \end{subfigure}
    \caption{Flight time and total energy for a representative mission.}
    \label{fig:sample_flight_time_energy}
\end{figure}
    
\begin{figure}[b]
\centering
    \begin{subfigure}{0.65\columnwidth}
        %\vspace{-1em}
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/sample_mission_legend.png}
        %\vspace{-2.8em}
        \vspace{-1.8em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.44\columnwidth}
        \centering
        \includegraphics[valign=t, trim=0 0 0 10, clip, width=\linewidth]{figs/sample_mission_average_velocity_zone.png}
        \vspace{-0.5em}
        \caption{Velocity across zones.}
        \label{fig:sample_flight_avg_velocity}
    \end{subfigure}
    \begin{subfigure}[t]{0.55\columnwidth}
        \centering
        \includegraphics[valign=t, trim=0 0 0 5, clip, width=\linewidth]{figs/sample_mission_dist_planning.png}
        \caption{Distance travelled and variable impact.}
        \label{fig:sample_flight_dist_planning}
    \end{subfigure}
    \caption{Velocity, distance, and planning metrics for a representative mission.}
    \label{fig:sample_mission_mission_metrics}
\end{figure}

%\begin{comment}
%\begin{figure*}[t]
%    \begin{subfigure}{0.7\textwidth}
%         \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figs/sample_mission_legend.png}
%        \label{fig:sample_legend}
%        \vspace*{-1.7em}
%    \end{subfigure}
%    
%    \begin{subfigure}[t]{0.32\textwidth}
%        \includegraphics[valign=t, trim=0 0 0 0, clip, width=\linewidth]{figs/sample_mission_flight_time_energy.png}
%   \caption{Mission metrics.}
%   \label{fig:sample_flight_time_energy}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.25\textwidth}
%        \includegraphics[valign=t, trim=0 0 0 0, clip, width=\linewidth]{figs/sample_mission_average_velocity_zone.png}
%   \caption{Average velocity across zones.}
%   \label{fig:sample_flight_avg_velocity}
%    \end{subfigure}
%    \begin{subfigure}[t]{0.33\textwidth}
%        \includegraphics[valign=t, trim=0 0 0 0, clip, width=\linewidth]{figs/sample_mission_dist_planning.png}
%     \caption{Distance travelled and the variables impacting it.}
%    \label{fig:sample_flight_dist_planning}
%    \end{subfigure}
%    \caption{Mission level metrics for a representative mission.}
%    \label{fig:sample_mission_mission_metrics}
%\end{figure*}
%\end{comment}

\begin{figure*}[t!]
\centering
    \begin{subfigure}[b]{0.95\textwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/boxplot_precision_volume_legend.png}
         \vspace*{-1.4em}
    \end{subfigure}
    
\hspace{-2em}
    \begin{subfigure}[b]{0.24\textwidth}
         \vspace{-1.5em}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/pc_res_decision_based_small.png}
         \vspace{-1.5em}
        \caption{Zone precision variations.}
        \label{fig:precision_boxplot}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
    \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/precision_dynamic_time_progression_small.png}
         \vspace{-1.5em}
        \caption{RoboRun precision over time.}
        \label{fig:precision_dynamic_time_prog}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
         \vspace{-1.5em}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/pc_res_decision_based_small.png}
         \vspace{-1.5em}
        \caption{Zone volume variations.}
        \label{fig:volume_boxplot}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
         \vspace{-1.5em}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/volume_dynamic_time_progression_small.png}
         \vspace{-1.5em}
        \caption{RoboRun volume over time.}
        \label{fig:volume_dynamic_time_prog}
    \end{subfigure}
    \caption{Variation of precision and volume across two designs.}
    \label{fig:precision_volume_SA}
\end{figure*}
  
\begin{figure*}[h!]
    \begin{subfigure}[b]{0.66\columnwidth}
     \vspace{-1.5em}
    \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/ee_latency_decision_based.png}
         \vspace{-1.5em}
        \caption{Zone latency variations.}
        \label{fig:latency_boxplot}
    \end{subfigure}
    \begin{subfigure}[b]{1.32\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/stage_breakdown_combined_time_progression_SA.png}
       \vspace{-1.5em}
        \caption{RoboRun (left) vs baseline (right) latency breakdown.}
        \label{fig:time_breakdown_dynamic_static}
    \end{subfigure}
    \caption{Impact of heterogeneity drivers, i.e. precision and volume, on end-to-end latency, across two designs. PC denotes point cloud, OM denotes OctoMap, PS denotes Path Smoother, and comm denotes communication.}
    \label{fig:ee_latency_SA}
\end{figure*}

\textit{Velocity(v):} 
Reducing flight time requires increasing velocity. RoboRun improves velocity by more than 4.6X (from 0.43~m/s to 2.01~m/s) by adapting the space precision and volume to the zone it is traveling in (Figure~\ref{fig:sample_flight_avg_velocity}). %By lowering the resolution and volume when possible, the drone lowers its end-to-end latency allowing for faster flights.    
% For spatial-aware, each zone's velocity is impacted by its congestion. 
Zone B's low congestion relaxes precision demands, decreasing latency and enabling higher velocity than in the congested zones A and C. We see a 4.6X velocity difference across the zones. 
In contrast, the baseline maintains a constant lower velocity, ignoring space demands. Note that even within the highly congested zones, RoboRun maintains a higher average velocity than the baseline by exploiting the heterogeneity in zones.

% Velocity of each zone impacts the time spent in it (Figure ~\ref{fig:sample_mission_mission_metrics}). Spatial-aware spends the least amount of time in zone B despite this zones larger size. This indicates that spatial-aware reduces distance impact when possible. In contrast spatial-oblivious spends most of its time in zone B since it maintains a fixed velocity throughout. 

% \textit{Travelled Distance (d):} Spatial-aware design negatively impacts the distance travelled by as much 1.3X. 
\textit{Distance Travelled (d):} Despite reducing the overall flight time, RoboRun increases the total distanced traveled by 1.3X (from 902~m to 1189~m) (Figure~\ref{fig:sample_flight_dist_planning}, left). Two factors cause this effect. First, lowering precision reduces (the drone’s perception of) the overall free space to plan within, and hence results in less optimal plans. Second, this reduction sometimes causes free space to be misclassified as occupied causing the drone to deviate from its path dodging inflated obstacles. Figure~\ref{fig:sample_flight_dist_planning}, far right shows the average optimality of generated trajectories across the two designs. Optimality is calculated by normalizing the generated trajectory length to the straight-line trajectory length, which is the shortest possible path between two points. Higher values indicate more deviation from this direct path and are undesirable. %and hence are undesirable. As seen, 
On average, RoboRun generates trajectories 1.5X worse than the straight-line path. Figure~\ref{fig:sample_flight_dist_planning}, middle, shows that RoboRun requires re-planning as much as 6X more frequently than the baseline (from 7 to 43 re-plans), due to the previously mentioned free space misclassification.

\textbf{Zone-based Metrics:}
Here we detail the differences in computation/communication between the two designs (Figures~\ref{fig:precision_volume_SA},~\ref{fig:ee_latency_SA}). %shedding light on the observed mission level (physical) discrepancies. 
First, we demonstrate zone level differences and then discuss discrepancies at the level of individual decisions. %by decision basis for a closer look.
%\red{static\_1 experiemenet 1}


%\begin{comment}
%\begin{figure*}[ht!]
%\centering
%    \begin{subfigure}{0.66\columnwidth}
%        \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/pc_res_decision_based.png}
%        \caption{Zone precision variations.}
%        \label{fig:precision_boxplot}
%    \end{subfigure}
%    \begin{subfigure}{0.66\columnwidth}
%    \centering
%     \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/precision_dynamic_SA.png}
%    \caption{Spatial aware precision over time.}
%    \label{fig:precision_dynamic_time_prog}
%    \end{subfigure}
%    \begin{subfigure}{0.66\columnwidth}
%   \centering
%      \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/precision_static_SA.png}
%    \caption{Spatial oblivious precision over time.}
%    \label{fig:precision_static_time_prog}
%    \end{subfigure}
%    
%    \begin{subfigure}{0.66\columnwidth}
%   \centering
%    \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/total_volume_decision_based.png}
%    \caption{Zones volume for spatial-aware/-oblivious.}
%    \label{fig:volume_boxplot}
%    \end{subfigure}
%   \begin{subfigure}{0.66\columnwidth}
%        \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/volume_dynamic_SA.png}
%        \caption{Spatial aware volume over time.}
%        \label{fig:volume_dynamic_time_prog}
%    \end{subfigure}
%    \begin{subfigure}{0.66\columnwidth}
%        \centering
%       \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/volume_static_SA.png}
%        \caption{Spatial oblivious volume over time.}
%        \label{fig:volume_static_time_prog}
%    \end{subfigure}
%  
%  \begin{subfigure}{0.66\columnwidth}
%     \centering
%    \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/ee_latency_decision_based.png}
%    \caption{Zone latency variations.}
%    \label{fig:latency_boxplot}
%    \end{subfigure}
%  \begin{subfigure}{0.66\columnwidth}
%        \centering
%        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/stage_breakdown_dynamic_SA.png}
%        \caption{Spatial aware computation (red shade) communication (blue shade with comm suffix) breakdown.}
%        \label{fig:time_breakdown_dynamic}
%    \end{subfigure}
%      \begin{subfigure}{0.66\columnwidth}
%    \centering
%    \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/stage_breakdown_static_SA.png}
%    \caption{Spatial oblivious computation/communication breakdown.}
%    \label{fig:time_breakdown_static}
%    \end{subfigure}
%  
%    
%       \caption{Variation of heterogeneity drivers, i.e., precision and volume, across two designs and their impact on end to end latency.}
%    
%
%      \label{fig:precision_SA}
%\end{figure*}
%\end{comment}

%\begin{comment}
%\begin{figure*}[h!]
%\hspace{-2em}
%\centering
%    \begin{subfigure}[b]{0.63\columnwidth}
%         \vspace{-1.5em}
%        \centering
%        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/pc_res_decision_based.png}
%         \vspace{-1.5em}
%        \caption{Zone precision variations.}
%        \label{fig:precision_boxplot}
%    \end{subfigure}
%    \begin{subfigure}[b]{1.29\columnwidth}
%    \centering
%        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/precision_combined_time_progression_SA.png}
%         \vspace{-1.5em}
%        \caption{RoboRun precision over time.}
%        \label{fig:precision_dynamic_static_time_prog}
%    \end{subfigure}
%    \caption{Variation of precision across two designs.}
%    \label{fig:precision_SA}
%\end{figure*}
%    
%\begin{figure*}[h!]
%    \begin{subfigure}[b]{0.66\columnwidth}
%    \vspace{-1.5em}
%    \centering
%        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/total_volume_decision_based.png}
%       \vspace{-1.5em}
%        \caption{Zone volume for RoboRun and baseline.}
%        \label{fig:volume_boxplot}
%    \end{subfigure}
%    \begin{subfigure}[b]{1.32\columnwidth}
%        \centering
%        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/volume_combined_time_progression_SA.png}
%        \vspace{-1.5em}
%        \caption{RoboRun volume over time.}
%        \label{fig:volume_dynamic_static_time_prog}
%    \end{subfigure}
%    \caption{Variation of volume across two designs.}
%    \label{fig:volume_SA}
%\end{figure*}
%\end{comment}



\textit{Precision Changes:}
RoboRun captures the heterogeneous precision demands of different zones, as shown in Figure~\ref{fig:precision_boxplot}.
RoboRun captures the greater heterogeneity of zones A/C with a significant variation in precision (top of the third and first quartiles are at 4.8 (m) and 0.6 (m), respectively). Zone B's box is small, reflecting its homogeneity. In contrast, the baseline has a small box (only containing 0.3 (m)) throughout the mission, ignoring space changes. RoboRun's bottom whiskers match those of the baseline, indicating the need for this worst-case precision.


%Here you can see how the bottom whisker for the spatial-aware design matches the value of the spatial-oblivious design indicating the need for this worse-case resolution. That said, the spatial-aware design often does not use this worst case precision and often uses a much lower precision allowing for lower computational latency and faster flight. This is most apparent in Zone B where on average the spatial-aware design uses a \red{TBD}X lower precision.
% quantifies the precision variability per zone for the two designs. Boxe's top/bottom delimit the precision's first/third quertile and the middle line shows the median. Spatial-aware captures higher heterogeneity of A/C zones with a bigger precision variation (box top and bottom are at 4.8 (m) and 0.6 (m)). Zone B's box is small reflecting its homogeneity. In contrast, spatial-oblivious has a small box (only containing 0.3 (m)) throughout the mission ignoring space changes. Note that the bottom whiskers for the spatial-aware matches those of spatial-oblivious indicating the need for this worse-case resolution.

Figure~\ref{fig:precision_dynamic_time_prog} shows these precision (Y-axis) changes at the decision level over time (X-axis) for RoboRun. Zones are delimited using dashed lines with zones A, B, C mapped to left, middle, and right. While the baseline uses a constant precision of 0.3 (m), RoboRun captures heterogeneity within the zones (smaller variations of 350 (s) to 500) and the differences across zones (larger variations of 100(s) to 150 (s)).
% For spatial-aware design, as the drone starts leaving zone A's high congestion (around 100 seconds) and nears zone A/B borders(around 150 seconds), voxel sizes are gradually increased from 0.3 (m) to 9.8 (m) reflecting the gradual congestion reduction in the environment. We see the opposite trend at around time 290 (s) when the drone starts entering zone C. Note that similar ascent/decent behavior is observed while we are deep within each zone. For example, between time 350 (s) and 500(s), we see many variations showing the captured heterogeneity within zone C. However, these variations are not as drastic and sharp as what we observe at zone borders since that's when the most congestion drop occur. In contrast, spatial-oblivious design maintains its highest precision of .3 (m) through out the mission.

% \begin{comment}
% \begin{figure}[t!] 
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/volume_dynamic_SA.png}
%         \caption{Variation in the volume for out spatial-aware design.}
%         \label{fig:volume_dynamic_SA}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/volume_static_SA.png}
%         \caption{Variation in the volume for out spatial-oblivious design..}
%         \label{fig:volume_static_SA}
%     \end{subfigure}
% \caption{Spatial-aware design adjusts its volume according to the space characteristics and the drone's budget. As seen, in congested areas the volume is lowered because the high precision demand impose high response time. Hence, to meet the time budget, it lowers the volume to counter balancing the precision effect. In contrast, a spatial-oblivious design does not adjusts its volume}
% \label{fig:res_quan}
% \end{figure}




% \begin{figure}[ht!]
% \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[trim=0 0 0 0, clip, height=1.5in]{figs/pc_res_decision_based.png}
%     \caption{Point cloud resolution.}
%     \label{fig:precision_boxplot}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%   \centering
%   \includegraphics[trim=0 0 0 0, clip, height=1.5in]{figs/octomap_volume_integrated_decision_based.png}
%     \caption{Space volume integrated in to octomap.}
%     \label{fig:volume_boxplot}
%     \end{subfigure}
%       \caption{Variation of point cloud resolution and octomap volume
%       across different zones. }
%       \label{fig:precision_SA}
% \end{figure}



% \begin{figure}[t!] 
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/end_to_end.png}
%         \caption{Variation in the end to end latency for out spatial-aware design.}
%         \label{fig:precision_dynamic_SA}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/end_to_end_latency_static_SA.png}
%         \caption{Variation in the end to end latency for out spatial-oblivious design..}
%         \label{fig:precision_static_SA}
%     \end{subfigure}
 
% \caption{Our Spatial-aware design adjusts its response time according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial-oblivious design does not adjusts its precision}
% \label{fig:res_quan}
% \end{figure}
% \end{comment}

\textit{Volume Changes:}
RoboRun also captures the heterogeneity in the volume processed, while the baseline must use a mostly constant\footnote{Although the baseline uses a constant volume, occlusions caused by obstacles along with the limitations of our operators results in a small variability.}, smaller volume due to its high worst-case precision requirement (Figure ~\ref{fig:volume_boxplot}). This allows RoboRun to explore larger areas of space while planning. We can see a much higher variation in the volume processed in zones A and C, accounting for the greater heterogeneity in the environment. Zone B's higher median is caused by its relaxed precision demands and hence, higher budget/volume affordability.
% reflects zones A/C heterogeneity with bigger variation in its volume processed (Figure ~\ref{fig:volume_boxplot}). These variations are mainly caused by frequent re-planning which requires extra volume to be processed. Zone B's higher median is caused by this zone's relaxed precision demands and hence higher budget/volume affordability. In contrast, spatial-oblivious imposes a high precision throughout and hence lowering its volume affordability. In addition, this design ignores space changes always imposing almost the same volume as shown with small boxes. Note by modulating the volume smartly, the volume of space processed by spatial-aware almost always stays above its counter part part allowing smarter planning/perception. 

Figure~\ref{fig:volume_dynamic_time_prog} shows the volume processed (Y-axis) by RoboRun as the mission progresses (X-axis). Each spike signifies an occurrence of re-planning. RoboRun modulates the spikes (based on the precision demanded/volume afforded within the budget), whereas the baseline keeps them fixed and short as it can not afford more volume.
For RoboRun, zone B's increasing trend in volume is due to map accumulation. Note that although the accumulation continues into zone C, its high congestion limits the drone's budget, restricting the map that can be afforded. 
The baseline also experiences this trend, but its limited volume affordability cuts it off quickly.


% \begin{comment}
% \textit{occlusion:} Obstacles block drone's FOV and hence reduce the volume of space sampled by sensors. Simply put, number/size of and distance to obstacles impact the amount of sampled space volume. This factor which is imposed by environment impacts the perception stage for both spatial-aware and oblivious designs although spatial-oblivious does incorporate this variation into its budget and hence can not take advantage of it. 

% \textit{precision bloat:} lowering precision (i.e., increasing voxel sizes), bloats the map volume. Simply put, doubling precision, increases each voxel cube by 8 times which specifically bloats the map's outer surface. Note this negatively impacts map fidelity as the bloated (perceived) obstacles leave less free space to navigate within. This factor impacts all stages of spatial-aware design.

% \textit{time budget:} Having more budget allows for a bigger space volume to be processed. This factor impacts  all stages of spatial-aware design.

% \textit{control-flow path:} The amount of space processed by the planning stage depends on the need for planning in the first place. If no planning is required, this space is minimal and vice versa. This environmentally imposed factor impacts the planning stage of both spatial-aware and oblivious design. 

% The combination of all above factors impact the space volume processed for each stage. Here we describe these impact specifically for our perception stage, leaving the rest to the reader.

%  Our spatial-aware design responds to zones with higher heterogeneity, i.e., zones A and C,  with a bigger variation (bigger box size) as shown in box plot blah. Zone B shows the biggest volume and smallest variation. the former is due to the combination of no-occlusion and precision bloat where as the latter is only imposed by time budget. Concretely, constant precision and no occlusion leaves time budget variations (imposed by our run-time) responsible for the variations observed.  Zone A and C have smaller volume and bigger variations due to compounding impacts of all factors mentioned above. Note that spatial-oblivious design also sees a variation across zone although only imposed by environment occlusion. This design can not take advantage of the environment provided variation since it assumes a fix time-budget throughout. \end{comment}
 

% \begin{comment}
% \textit{Response Time Changes}
% Our Spatial-aware design adjusts its response time to meet the space demands and time budget. As seen, in congested Zones, i.e., A and C, that drone requires high precision, response time is increased whereas it is gradually lowers it as it enters and increase it as it exits zone B. In contrast spatial-oblivious design maintains its design time response time through out the mission. Note that the spikes in both figures signify that a planner has been triggered to generate a trajectory around obstacles.

% Figure blah shows the response time standard deviation and average min and max through each zone for the two designs. As seen congested areas \red{use the graph to write something}



% Figure blah shows the precision standard deviation and average through each zone for the two designs. As seen congested areas \red{use the graph to write something}

% \begin{figure}[t!] 
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/ee_latency_decision_based.png}
%         \caption{latency comparison.}
%         \label{fig:computation_dynamic_SA}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/PERF_COUNT_HW_INSTRUCTIONS_decision_based.png}
%         \caption{hardware instructions comparison}
%         \label{fig:precision_static_SA}
%     \end{subfigure}
% \caption{Our Spatial-aware design adjusts its latency associated with each stage according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial-oblivious design does not adjusts its precision}
% \label{fig:res_quan}
% \end{figure}
% \end{comment}
\begin{comment}
\begin{figure*}[t!] 
    \centering
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/computation_breakdown_dynamic_SA.png}
        \caption{RoboRun computation break-down.}
        \label{fig:computation_dynamic_time_prog}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/computation_breakdown_static_SA.png}
        \caption{Spatial oblivious computation break-down.}
        \label{fig:computation_static_time_prog}
    \end{subfigure}
   \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/normalized_comp_breakdown_per_decision.png}
        \caption{Average latency contribution of each computation stage.}
        \label{fig:computation_hotspot}
    \end{subfigure}
   
  
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/communication_breakdown_dynamic_SA.png}
        \caption{RoboRun communication break down.}
        \label{fig:communication_dynamic_time_prog}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/communication_breakdown_static_SA.png}
        \caption{Spatial oblivious communication break-down.}
        \label{fig:communication_static_time_prog}
    \end{subfigure} 
     \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/normalized_comm_breakdown.png}
        \caption{Average latency contribution of each communication stage.}
        \label{fig:communcation_hotspot}
    \end{subfigure}

\caption{RoboRun adjusts its latency associated with each stage according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial oblivious design does not adjusts its precision.}
\label{fig:res_quan}
\end{figure*}
\end{comment}





\textit{End-to-End latency:}
The compounding impact of precision and volume varies the end-to-end latency for both designs. 
RoboRun maintains an end-to-end latency less than the baseline's throughout most of the mission (Figure~\ref{fig:latency_boxplot}) with a median latency reduction of up to 11X. However, it does incur some high latency outliers as it aggressively reduces precision and consumes volume causing slowdowns of up to 1.2X. 
% Top of the boxes for spatial-aware are always lower than their counterparts, and further theirs medians are sped up by as much as 11x. However, spatial-aware incurs some high latency outliers (shown with the top whisker's) due to its aggressive resolution reduction and volume consumption (both impacting the planning generation time). These slow-downs can be as much as 1.2X.  

RoboRun also better matches the environment with almost no variation in the homogeneous zone (0.15 seconds for zone B) and high latency variations in the heterogeneous zones (10 and 12.5 seconds for zones A and C respectively). In contrast, the baseline maintains a smaller change across all zones (max of 5.4 seconds). Note that the baseline cannot use its variations toward velocity improvement due to its fixed budget.
% Spatial-aware is in tune with space variations. More heterogeneous zones (A/C) incur a higher latency variation (10 and 12.5 seconds respectively) than the homogeneous zone B (with 0.15 seconds). In contrast, spatial-oblivious maintains a smaller variation across zones (highest of 5.4 seconds). Note that spatial-ware variations (caused by the need for re-planning) can not be used toward velocity improvement due to its fix imposed budget.

Figure ~\ref{fig:time_breakdown_dynamic_static} shows both designs' end-to-end latency broken down by computation (shades of red) and communication (shade of blue) stages. Note the baseline has a largely uniform computation/communication profile (right graph) in comparison with RoboRun (left graph). For RoboRun, spikes can be categorized into high-precision/low-volume (e.g. point X), low-precision/high-volume (e.g. point Y), and mid-precision/mid-volume (e.g. point Z) moments. The first cluster (perception heavy) occurs in high congestion/high goal visibility/accessibility areas. The second (planning heavy) occurs in low congestion/low goal visibility and the third somewhere in between. RoboRun responds to an area's demand/heterogeneity accordingly in contrast to baseline.

Both designs pay a fixed 210 (ms) point cloud latency, and RoboRun pays an extra 50 (ms) runtime latency. However, as we have shown, by saving latency from other stages, this latency cost almost never impacts this design's overall benefit.

\begin{figure}[t]
\centering
 \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/normalized_time_breakdown.png}
        \caption{Average latency contribution of each pipeline stage.}
        \label{fig:computation_hotspot}
\end{figure}

%highly congested areas when no obstacle is intersecting drone's trajectory. Second cluster (planning heavy) occurs when drone is in low congestion areas but has bad visibility/accessibly to the goal, and third covers scenarios in between. 



%occur shows a perception light/planning heavy moment. These moments occur when drone is in low congested areas but with bad visibility/accessibility to the goal. Point C shows both perception and planning under pressure.


%though are caused by either a resolution drop, a volume rise or a combination of the two. Points A, B and C show high-res/low-volume, low-resolution/high-volume and mid-resolution/mid-volume points. In contrast, spikes in the spatial-oblivious design shown in Figure~\ref{fig:latency_static_time_prog} are only caused by the need for re-planning. They are also almost identical indicating fix design choices.



% \begin{comment}
% The spikes in the graph b show the need for re-planning. As seen zone A and C are populated with the spikes. Spatial-aware design modulates the height of these spikes however by controlling the precision and volume when it can lowering the end-to-end latency for making a decision. As shown these spikes can be as small as blah second and as big as blah second. On the other hand, the spikes for the spatial-oblivious design has very little variations since fix budget for all the stages are allocated regardless. 
% \end{comment}


% \begin{comment}
% Spatial-aware design maintains its computation latency bellow its counterpart through out most of the mission. As shown, top of the boxes for spatial-aware is always lower, and further medians are sped up by as much as blah x. However, spatial-aware incurs some latency outliers (shown with the top whisker's) due to its aggressive resolution reduction which impacts planning generation time. These slow-down can be as much as blah x.  

% Spatial-aware is in tune with space variations. As shown, more heterogeneous zones such as A and C incur a higher latency variation (blah \red{radhika} seconds) than the homogeneous zone B (with blah \red{radhika} seconds). In contrast, spatial-oblivious design maintains a smaller variation across zones (highest of blah seconds). Note this variation is caused by the need for re-planning when the trajectory is intersected by an obstacle. However, since this design assume a fix budget, it can not turn such variations toward velocity improvements.
% \end{comment}

%\textit{Computation Break Down:}
%In this section we break down the computational latency of each stage in the navigation pipeline for this mission as shown in Figures ~\ref{fig:computation_dynamic_SA} and~\ref{fig:computation_static_time_prog}. The spatial-oblivious design has a uniform perception latency and a relatively uniform planning latency with mostly small variations caused by the stochastic nature of the planner. On the other hand, the spatial-aware design tunes the time spent per stage depending on space demands. Note that while the spatial-aware design incurs an extra run-time fixed  latency, overall it is able to greatly reduce the total computational latency of the navigation pipeline freeing up compute resources for other tasks. 

%For the spatial-aware design we can also tie particular computational demands to the environment. Point A shows a perception heavy/planning light moment. These moments occur when drone is in highly congested areas but no obstacle is currently intersecting its trajectory. Point B shows a perception light/planning heavy moment. These moments occur when drone is in low congested areas but with bad visibility/accessibility to the goal. Point C shows both perception and planning under pressure.

% Spatial-aware tunes time spent per stage depending on space demands. Figure ~\ref{fig:computation_dynamic_SA} shows each stage's latency with layers from bottom to top following the control flow order, i.e., front-end to back-end. Point A shows a perception heavy/planning light moment. These moments occur when drone is in highly congested areas but no obstacle is currently intersecting its trajectory. Point B shows a perception light/planning heavy moment. These moments occur when drone is in low congested areas but with bad visibility/accessibility to the goal. Point C shows both perception and planning under pressure.  Note that spatial-oblivious impose a uniform perception pressure with planning causing spikes sometimes (Figure ~\ref{fig:computation_static_time_prog}). 

% A fix latency point cloud generation latency is paid by both of the designs. In addition, spatial-aware incurs an extra run-time fix latency. However, as we have shown, by saving latency from other stages, this latency almost never impacts the over all benefit of this design.

Figure ~\ref{fig:computation_hotspot} shows what portion of the end-to-end latency each stage consumes. For RoboRun the bottleneck shifts depending on the precision and the volume required. Zone B's low congestion shifts the bottleneck toward runtime and point cloud since small voxel sizes reduce OctoMap's processing time, and in general, no re-planning is needed. On the other hand, congested areas within zones A and C distribute the computation more evenly across all stages. In contrast, the baseline always distributes the computation the same way, pressuring OctoMap. RoboRun has a more balanced pipeline in high congestion areas when the system is under high pressure.% and hence is a better design. 


% \begin{comment}

% \begin{figure}[t!] 
  
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/communication_breakdown_decision_based.png}
%         \caption{Comparison of hardware instruction count across zones.}
%         \label{fig:precision_static_SA}
%     \end{subfigure}
% \caption{Our Spatial-aware design adjusts its latency associated with each stage according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial-oblivious design does not adjusts its precision}
% \label{fig:res_quan}
% \end{figure}
% \end{comment}

% \begin{comment}
% Spatial-aware design maintains its communication latency bellow its counterpart through out most of the mission. As shown, top of the boxes for spatial-aware is always lower, and further medians are sped up by as much as blah x. However, spatial-aware incurs some latency outliers when a map with bigger volume can be afforded. In the worse-case scenario, spatial-aware spends blah x more on communicating the maps (with a higher volume) than its counter part. 


% Spatial-aware is more in tune with space variations. As shown, more heterogeneous zones such as A and C incur a higher latency variation (blah \red{radhika} seconds) than the homogeneous zone B (with blah \red{radhika} seconds). In contrast, spatial-oblivious design maintains a smaller variation of blah second. The gradual increase in medians for spatial-oblivious design is resulted from the accumulated map. As the drone moves through space, it accumulates more maps. In the case of spatial-oblivious design, a cap of 15000 is reached somewhere in the middle of zone one. This can be seen in figure blah as the latency platos after. The higher variation in this zone is also caused by such accumulation where as zone two sees a smaller variation with the platoed map. 
% \end{comment}

%\textit{Communication Break Down:}
%Figures~\ref{fig:communication_dynamic_time_prog} and~\ref{fig:communication_dynamic_time_prog} show the communication latency between the different stages of the navigation pipeline. For the spatial-aware design spikes show moments (mainly in zones A and C) when higher precision/bigger maps are communicated. For these spikes, most of the processing is spent on passing the map to the planner. On the other hand, the spatial-oblivious design is bottlenecked at first by the point cloud and then gradually by the map as the accumulated map expands. Finally we note that the spatial-aware design has a more evenly distributed though less balanced communication signature (Figure ~\ref{fig:communcation_hotspot}). 


% \begin{comment}
% \begin{figure}[t!] 
    
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/datamovement_dynamic_SA.png}
%         \caption{datamovement for spatial-aware design.}
%         \label{fig:computation_dynamic_SA}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/datamovement_static_SA.png}
%         \caption{datamovement for spatial-oblivious design}
%         \label{fig:precision_static_SA}
%     \end{subfigure}
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/cache_references_only_dynamic_SA.png}
%         \caption{memory foot print for spatial-aware design.}
%         \label{fig:computation_dynamic_SA}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/cache_references_only_static_SA.png}
%         \caption{memeory foot print for spatial-oblivious design}
%         \label{fig:precision_static_SA}
%     \end{subfigure}
    
% \caption{Our Spatial-aware design adjusts its communication load associated with each stage according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial-oblivious design does not adjusts its precision}
% \label{fig:res_quan}
% \end{figure}

% \end{comment}
\begin{comment}
\begin{figure}[t!] 
    
     \centering
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/PERF_COUNT_HW_INSTRUCTIONS_decision_based.png}
        \caption{datamovement for spatial-aware design.}
        \label{fig:computation_dynamic_SA}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/CACHE_REFERENCES_decision_based.png}
        \caption{memory foot print}
        \label{fig:precision_static_SA}
    \end{subfigure}
\caption{RoboRun adjusts its latency associated with each stage according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial-oblivious design does not adjusts its precision}
\label{fig:res_quan}
\end{figure}
\end{comment}
%\subsection{Modeling} Behzad/Jon

% \begin{comment}
% \subsection{Zone base Analysis}
% In this section, we show the accumulative impact of fine grain results presented above for each zone. Concretely, we present system level metrics such as decision rate, hw memory instruction and further their impact on motion level metrics such as velocity and time spent per zone.
% Note that we normalize our system metrics to the size of each zone (concretely the diagonal distance) to cancel out the discrepancy in their sizes. This is because, intuitively speaking, more computation computation is necessary when a longer distance is travelled. Hence, normalizing to distance shifts the focus toward space difficulty rather than space distance. As we show, the space heterogeneity gets reflected in the computation and communication of the spatial-aware design whereas the spatial-oblivious design behaves as if the entire space is homogeneous. 

% Figure blah shows the variation in number of hw instructions and memory bytes processed within each zone (normalized to the zone size). As seen, more congested zones take 

% \begin{figure}[t]
% \includegraphics[width=\columnwidth]{figs/end_to_end_results.png}
% \caption{End to End results}
% \label{velocity_drivers}
% \end{figure}

% \end{comment}



% \begin{comment}
% \begin{figure}[t!] 
%     \begin{subfigure}{0.43\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/flight_time_heat_map.png}
%         \caption{datamovement for spatial-aware design.}
%         \label{fig:computation_dynamic_SA}
%     \end{subfigure}
%     \begin{subfigure}{0.43\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/total_energy_consumed_heat_map.png}
%         \caption{memory foot print}
%         \label{fig:precision_static_SA}
%     \end{subfigure}
% \caption{Our Spatial-aware design adjusts its latency associated with each stage according to the budget and space needs. High precision areas such as A and C impose higher latency whereas B does not. In contrast, a spatial-oblivious design does not adjusts its precision}
% \label{fig:res_quan}
% \end{figure}
% \end{comment}



\begin{comment}
\begin{figure}[t]
\includegraphics[width=\columnwidth]{figs/varying_goal_distance.png}
\caption{Impact of goal distance variation the mission.}
\label{fig:goal_sensitivity_analysis}
\end{figure}
\end{comment}
%\begin{table}[]
%\resizebox{0.47\textwidth}{!}{
%\begin{tabular}{|l|cccccc|}
%\hline
%                   & \multicolumn{6}{c|}{Environment Knobs}                                                                             \\
%Mission Metrics    & \multicolumn{2}{c}{Spread}           & \multicolumn{2}{c}{Congestion}        & \multicolumn{2}{c|}{Goal Distance} \\ \cline{2-7} 
%                   & Dynamic & \multicolumn{1}{c|}{Static} & Dynamic & \multicolumn{1}{c|}{Static} & Dynamic          & Static          \\ \hline
%Flight Time        & 0.38    & \multicolumn{1}{c|}{0.16}   & 0.39    & \multicolumn{1}{c|}{0.18}   & 0.24             & 0.94            \\
%Total Energy       & 0.35    & \multicolumn{1}{c|}{0.14}   & 0.40    & \multicolumn{1}{c|}{0.16}   & 0.19             & 0.87            \\
%Distance Travelled & 0.07    & \multicolumn{1}{c|}{0.16}   & 0.18    & \multicolumn{1}{c|}{0.18}   & 0.74             & 0.93            \\
%Average Velocity   & -0.52   & \multicolumn{1}{c|}{-0.02}  & -0.36   & \multicolumn{1}{c|}{-0.00}  & 0.45             & 0.15            \\ \hline
%\end{tabular}}
%\caption{\label{tab:correlation_table} Pearson correlation coefficient values for different mission metrics versus environment difficulty knobs.}
%\end{table}







% \begin{comment}


% Figure \ref{environment_sensitivity} compares the impact of congestion (peak and spread) across the two designs. Note that  we limit our discussion to flight time since energy shows the same exact trend. X and Y axis denote congestion spread and peak respectively and the heat-map shows the relative flight-time variation normalized to the easiest setup, i.e., peak = .3 and spread = 40. Each value in the map is collected and averaged over 8 data points.

% Environment changes has a big impact on spatial-aware flight time. This can be observed with the severity with which colors change within the map. This indicates that spatial aware design reacts to space changes. Over all we see a 164\% flight time variation between the easiest and the hardest map. In contrast, spatial-oblivious design ignores space changes only reflecting a  small flight time variation of 24\%.

% Spatial-aware design shows almost equal sensitivity toward congestion peak and spread, 55\% and 53\%  respectively \footnote{These values are calculated by getting the average difference of last and first row for peak and the corresponding calculation over columns for spread}. This signifies that an efficient spatial-aware design must prioritize across both axis for optimal flights. Note that spatial-oblivious design shows a small 5\% and 11\% for its corresponding numbers.

% Congestion spread does not uniformly impact flight time across different congestion peaks. As shown, spread of 40 (first column) impacts flight time by as much as 50\% as we do a column walk from lower (.3) to higher (.6) congsetion. On the other hand, similar walk for the spread of 120 results in 65\% variation. Intuitively speaking, this means that the impact of congestion spread is more severe for higher congestion peaks. Similar relationship hold for peak and spread. This indicates that the compounding impact of congestion peak and spread can not be simply reduced to a linear relationship. 

% \enc{comment}















% \begin{comment}
% dynamic:
% (2.64 - 1.49) / 1.49 = 0.77
% (1.74 - 1.33) / 1.33 = 0.3
% (1.60 - 1.00) / 1.00 = 0.6
% (0.77 + 0.3 + 0.6) / 3 = 0.55
% average of rows: 55%
% average of columns: 53%
% static:

% row averages = [0.01 0.01 0.14]
% col averages = [0.08 0.04 0.22]
% average of row averages = 5%
% average of col averages = 11%
 
% \end{comment}
% \begin{figure}[t]
% \includegraphics[width=\columnwidth]{figs/performance_models.png}
% \caption{Cyber physical performance models.}
% \label{mission_metrics}
% \end{figure}


==> tex/roborun_design.tex <==
\section{RoboRun: A Spatial Aware Middleware}
\label{sec:roborun_design}
% To address the shortcomings of spatially-oblivious designs,
%In this paper, we proposespatial-awarecomputing, a cyber-physical co-design framework that exploits the synergy be-tween the robot’s heterogeneous environment and its computesubsystem

%To take advantage of spatial-aware cyber-physical co-design,
We present \textit{RoboRun}, a spatial aware middleware
that exploits the synergy between the robot’s heterogeneous environment and its compute subsystem. RoboRun
continuously assesses the external world's and MAV's internal demands, adjusting the computational resources accordingly. First, we discuss RoboRun's overall architecture and then detail its components. We implemented RoboRun on top of
Robot Operating System (ROS)~\cite{quigley2009ros}, which provides low-level inter-process communication libraries, and high level common robotics packages.

\subsection{RoboRun Overview} RoboRun uses a distributed design with three components: a governor, profilers, and operators (Figure ~\ref{fig:PPC_pipeline}, green blocks).  Briefly, the governor uses profilers to monitor the drone's internal and external states (e.g. velocity and obstacle density) and compute optimal time budget policies. 
As shown in the task flow (thick arrows) of Figure~\ref{fig:PPC_pipeline}, the governor sits towards the beginning of the pipeline generating policies as the sensory inputs arrive.
%(e.g., processed point cloud data) 
These policies are then passed to the precision and volume operators (thin dataflow arrows) for enforcement. 
In the following sections, we give details of each component. 



%uch applications typically consist of concurrent processes
%alled ``nodes,'' each of which runs a different part of the navigation
%ipeline.

%\red{behzad, cut down after jon gives you the figure}
%\textbf{Task-Flow:} Figure ~\ref{fig:task_flow} shows the task flow associated with the navigation stack on left of the dotted line (as previously described in Section~\ref{sec:navigationPipeline}) with our runtime task flow on the right of the dotted line.
%In our dynamic design, the governor uses both a front end to determine the time budget, and a back-end to determine the precision and volume for the stages highlighted in yellow based on this budget (we will refer to these as the ``knob settings''). In contrast, a static design assumes a fixed budget (corresponding to fixed precision and volume) for all stages. We note that if the governor determines that there is not enough time budget to complete the computation with the minimum require precision and volume it will signal the control system to stop the drone.


% \begin{figure*}[t!] 
%     \centering
%     \begin{minipage}[b]{\columnwidth}
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_overall_arch.png}
%             \caption{Overall architecture}
%             \label{fig:overall_arch_2}
%         \end{subfigure}\\[\baselineskip]
%         \begin{subfigure}[b]{\linewidth}
%             \centering
%             \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_runtime_detail.png}
%             \caption{Detailed architecture}
%             \label{fig:over_archiecture}
%         \end{subfigure}
%     \end{minipage}
%     \hfill
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_runtime_taskflow.png}
%         \caption{Augmenting the navigation-stack task flow with our runtime.}
%         \label{fig:task_flow}
%     \end{subfigure}
% \caption{Our runtime overall architecture and taskflow}
% \label{fig:middleware_design}
% \end{figure*}

% \begin{figure}[b]
%     \centering
%     \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_runtime_detail.png}
%     \caption{Operator and governor task flow.}
%     \label{fig:op_archiecture}
% \end{figure}


% \begin{figure*}[b!]
%     \centering
%     \includegraphics[trim=0 0 0 -25, clip, width=.6\linewidth]{figs/operator_table.png}
%     \caption{Operator Table}
%     \label{fig:operator_table}
% \end{figure*}

\begin{table}[t!]
\centering
\small
\resizebox{.49\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Pipeline Stage}              & \textbf{Knobs}                 & \textbf{Description}                                   \\ \hline
\multirow{2}{*}{Perception}             & Volume                         & \begin{tabular}[c]{@{}c@{}}Space volume merge into map.\end{tabular}    \\ \cline{2-3} 
                                        & \multicolumn{1}{l|}{Precision} & \begin{tabular}[c]{@{}c@{}} Space precision merged into map.\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Perception to \\ Planning\end{tabular}} & Volume                         & \begin{tabular}[c]{@{}c@{}}Map's volume passed to planner.\end{tabular}               \\ \cline{2-3} 
                                        & \multicolumn{1}{l|}{Precision} & \begin{tabular}[c]{@{}c@{}}Map's precision passed to planner.\end{tabular}            \\ \hline
\multirow{2}{*}{Planning}               & Volume                         & \begin{tabular}[c]{@{}c@{}}Map's volume explored by planner.\end{tabular}                   \\ \cline{2-3} 
                                        & \multicolumn{1}{l|}{Precision} & \begin{tabular}[c]{@{}c@{}} Map's precision explored by planner.\end{tabular}           \\ \hline
\end{tabular}}
\caption{Operator Table. Knobs control their variables each iteration.}
\label{fig:operator_table}
\end{table}

% \begin{figure*}[ht!]
%     \centering
%     \includegraphics[trim=0 0 0 -25, clip, width=.6\linewidth]{figs/runtime_arch_flow/roborun_runtime_detail.png}
%     \caption{Detailed archiecture}
%     \label{fig:over_archiecture}
% \end{figure*}
\begin{figure}[ht]
    \centering
     \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_precision_op_detail.png}
        %\vspace{-1.5em}
        \caption{Precision Operator}
        \label{fig:prec_op_flow}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\linewidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_volume_op_detail.png}
        %\vspace{-1.5em}
        \caption{Volume Operator}
        \label{fig:vol_op_flow}
    \end{subfigure}
      \vskip\baselineskip
   \begin{subfigure}[b]{0.4\linewidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_profiler_detail.png}
       %\vspace{-1.5em}
        \caption{Profiler}
        \label{fig:prof_flow}
    \end{subfigure}
    \hfill
   \begin{subfigure}[b]{0.4\linewidth}
        \centering
        \includegraphics[trim=0 0 0 0, clip, width=\linewidth]{figs/runtime_arch_flow/roborun_gov_detail.png}
        %\vspace{-1.5em}
        \caption{Governor}
        \label{fig:gov_flow}
    \end{subfigure}
    \caption{Task flows of our runtime's components.}
    \label{fig:op_architecture}
\end{figure}


\subsection{Operators}
They enforce the precision and volume policies (Table~\ref{fig:operator_table}).
% Since the spatial reasoning computation is 
% spread across the navigation pipeline, our operators are also distributed across it. Concretely,
% point cloud, octomap, and planners each employ their own operators. 
%Table~\ref{fig:operator_table} lists all of our operators, and their placement and functionality in the navigation pipeline. 
Due to space limitations, we only provide an overview of each. %operator.

\textbf{Precision Operators:}
They enable accuracy-latency trade-offs by enforcing the precision of space processed. Environments with higher precision requirements incur greater computational latency and hence lower velocity.
%We deploy two precision operators, one for perception, one for planning. 

Point cloud (perception stage) precision is enforced by controlling the sampling distance between points. We grid the space into cells and map the points onto these cells using their coordinates. Finally, we reduce all of the points within a cell into a single average point (Figure~\ref{fig:prec_op_flow}). 
%Note nearest neighbors sampling policy will not work.
OctoMap (perception stage) precision is enforced by controlling the step size (voxel count) of the ray tracing step.
Perception to planning precision is enforced by sub-sampling and pruning the tree structure of the encoded map, and planning precision is enforced by modifying the raytracer, similar to OctoMap.   


%subsampling the map passed to the planning stage by the Octomap kernel. Since this map is encoded with various levels of resolution across different tree levels (\red{figure blah. jon show a octomap with 3 levels and mark the shallow to deep direction one one side and precision change on the other)}), this can simply by done by limiting the depth of our map queries. In addition, collision checking requires modifying raytracing as described above.

%\textbf{objective function and constraints \green{Jon}}

\textbf{Volume Operators:}
They enable volume-latency trade-offs by enforcing the volume of space processed. Processing a higher volume leads to better world modeling but requires higher computational latency and hence lower velocity. 

We deploy three volume operators from Table~\ref{fig:operator_table}, all following Figure~\ref{fig:vol_op_flow} task flow.
The first operator (perception stage) controls the volume of space added to the map. We sort the space (sequencer) based on the distance to the drone's trajectory, as closer points pose higher threats if containing obstacles. Sorted points are integrated one by one until their resulting volume exceeds the desired threshold (monitor).
%. while their added volume monitored and cut off once our desired threshold is reached (monitor).
%in order while the  based on this distance function and then monitor their  Then our monitor integrates the points in that order until we reach the maximum volume demanded by the governer. 
The second operator (perception to planning) controls the space volume communicated to the planner, limiting the planner's knowledge of the world.
Similarly, we sort the space based on the proximity to the drone (sequencer).  To do so, we prune the map, which is encoded in a tree, by selecting higher level trees (in the sorted order) until the threshold is reached (monitor).
%We To do so, we also use a sequencer (for prioritizing) and a monitor (for thresholding). Our ordering also prioritizing the space based on the vicinity to the drone. To do so, we prune the map by selecting higher level trees in the aforementioned order until the demand volume is reached.
The third operator (planning stage) controls the space volume explored by the planner. RRT* itself acts as a sequencer by sorting the points/paths within the explored space. We add a volume monitor to stop the search once it exceeds the volume.
%by the planner. This limits the amount of space explored by the planner as it generates its trajectory. In our design, a piecewise planner (RRT*) itself acts as a sequencer by prioritizing the points and paths within the space to explore. We introduce a volume monitor to stop the search once its exceeds the demanded volume.
\subsection{Profilers}
To adjust precision and volume knobs, environmental information, such as gaps between obstacles, and internal drone state, such as current velocity, are profiled from the sensors and navigation pipeline.
Profilers iterate and post-process each stage's data structures, e.g. point cloud array, tree map, and trajectory (Figure~\ref{fig:prof_flow}), to extract space characteristics (Table~\ref{fig:profiling_table}).

\subsection{Governor}
\label{subsec:governor}
The governor is responsible for allocating the time budget (deadline) for the end-to-end navigation pipeline and determining the correct precision and volume settings per stage to satisfy this budget and space demands (Figure~\ref{fig:gov_flow}). 

\subsubsection{Time Budgetting:}
The \textit{time budget} (processing deadline) is the maximum amount of time that can be spent processing an input while maintaining collision-free flight. 

% \begin{figure}[t!]
% \centering
% \includegraphics[trim=0 0 0 -25, clip, width=\linewidth]{figs/budgetting_algorithm.png}
% \caption{Budgeting algorithm for trajecotry/budgetting codesign.}
% \label{fig:budgetting_algorithm}
% \end{figure}

% \begin{figure*}[b!]
% \centering
% \includegraphics[trim=0 0 0 -25, clip, width=.6\linewidth]{figs/profiling_table.png}
% \caption{List of variables profiled and used by the governor to determine the end-to-end budget, each stage budget and further precision and volume accordingly}
% \label{fig:profiling_table}
% \end{figure*}

\begin{table}[]
\resizebox{.48\textwidth}{!}{%
\centering
\small
\begin{tabular}{|c|c|c|}
\hline
\textbf{Variable}            & \textbf{Profiled Pipeline Stage} & \textbf{Used For}       \\ \hline 
Gap between obstacles        & Point cloud               & Precision             \\ \hline
\begin{tabular}[c]{@{}c@{}}Closest obstacle, \\ closest unknown\end{tabular} & \begin{tabular}[c]{@{}c@{}}Point cloud,  \\ OctoMap, Smoother\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Precision, Volume, \\ Time budget\end{tabular}  \\ \hline
 Sensor, map volume        & Point cloud, OctoMap               & Volume                  \\ \hline
 Velocity, position             & Sensors                   & Time budget             \\ \hline
Trajectory             & Smoother                & Time budget             \\ \hline
\end{tabular}}
\caption{Profiler Table. These variables are collected by profilers.}
\label{fig:profiling_table}
\end{table}


\begin{comment}
\begin{table}[]
\centering
\small
\begin{tabular}{|c|c|c|}
\hline
\textbf{Variable}            & \textbf{Associated Stage} & \textbf{Used For}       \\ \hline
Gap between obstacles        & Point cloud               & Precision               \\ \hline
\begin{tabular}[c]{@{}c@{}}Distance to nearest \\ obstacle\end{tabular} & \begin{tabular}[c]{@{}c@{}}Point cloud, \\ Octomap\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Precision, \\ Time budget\end{tabular}  \\ \hline
Current sensor volume        & Point cloud               & Volume                  \\ \hline
Current map volume           & Octomap                   & Volume                  \\ \hline
Current velocity             & Sensors                   & Time budget             \\ \hline
Drone trajectory             & Smoothener                & Time budget             \\ \hline
Current drone position       & PID Control               & Time budget             \\ \hline
\begin{tabular}[c]{@{}c@{}}Distance to nearest \\ unknown\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Point cloud, \\ Octomap\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Visibility, \\ Time Budget\end{tabular} \\ \hline
\end{tabular}
\caption{List of variables profiled and passed to governor for time-budgeting and precision/volume tuning.}
\label{fig:profiling_table}
\end{table}
\end{comment}

The time budget depends on the space traversal velocity and space visibility. Equation~\eqref{eq:motion_model} \cite{liu2016high} shows the relationship between these variables, where $d$ is the space visibility, $v$ is space traversal velocity, and $d_{stop}(v)$ is the distance the MAV needs to stop at velocity $v$. The numerator specifies the minimum safe distance between an obstacle and the MAV given its velocity. The division by the denominator sets an upper bound on MAV's time budget to ensure collision-free flight. %it stays within this distance if drones continues with velocity v.  
$d_{stop}(v)$ is modeled by flying the drone with various velocities in simulation and measuring the stopping distance. Equation \ref{eq:d_stop} shows our model with <2\% MSE.

\begin{comment}
\begin{equation}
    \label{eq:motion_model}
    v_{max} = a_{max} \left( \sqrt{\delta t^2 + 2\frac{d}{a_{max}}} - \delta t \right).
\end{equation}
\end{comment}
\begin{equation}
    \label{eq:motion_model}
    \text{Time budget} = \frac{(d - d_{stop}(v))}{v}
\end{equation}

\begin{algorithm}[!t]
\begin{algorithmic}[1]
\caption{Time Budgeting Algorithm}
\label{fig:budgetting_algorithm}
\State $b_g \gets 0$
\State $b_r \gets \text{Equation}~\ref{eq:motion_model} \text{ at } W_0$
\For{$i = 1 \dots |W|$}
    \State $b_r \gets b_r - flightTime(i,i-1)$
    \State $b_l \gets \text{Equation}~\ref{eq:motion_model} \text{ at } W_i$
    \State $b_r \gets min(b_r,b_l)$
    \If{$b_r \leq 0$} \textbf{break}
    \EndIf
    \State $b_g \gets b_g + flightTime(i,i-1)$
\EndFor
\State \Return $b_g$
\end{algorithmic}
\end{algorithm}

\begin{equation}
    \label{eq:d_stop}
    d_{stop(v)}= -0.055*v^2 - 0.36*(v)+ 0.20
\end{equation}

Equation~\eqref{eq:motion_model} assumes a fixed velocity and visibility for the duration of the time budget. This can result in overly optimistic budgets as these variables can change. To improve this model, we derive an algorithm to take into account the instantaneous velocity and visibility, and the planned velocity and visibility for upcoming waypoints ($W$). Our algorithm computes the global\_budget ($b_g$) as a running sum. This ensures that at each waypoint, the duration of the flight from the previous waypoint and the local\_budget at that waypoint ($b_l$ computed using Equation~\eqref{eq:motion_model}) are considered.
With this, environment variations at all waypoints are accounted for ensuring safe flight. See Algorithm~\ref{fig:budgetting_algorithm} for more details.

% by takes its minimum against budget inherited from previous waypoints (stored in global\_budget). This ensures the point with the highest velocity/lowest visibility will determine the overall budget. Note that since drone travels between two waypoints, global\_budget needs to be decremented according to their time difference.
% The algorithm terminates once global\_budget plummets below zero, indicating that no further waypoint can be reached without the possibility of collision. At this point, accumulated\_budget contains the budget. 

\subsubsection{Solver:}
It determines the precision and volume required per stage to fit the budget while ensuring space demands are met.
The solver uses the profiled variable and the time budget.
%Profiled information  the time budget are used to determine the 
%Combining this with the end-to-end time budget,
%acquired from the time-budgetter, 
%the solver can then determine the 
%precision and volume for each stage.
%For example, as shown, the gap between obstacles is collected from the point cloud kernel and used to determine the precision for the octomap kernel.

%To find the operator (i.e, volume and precision) setting that meets the required deadlines while exploiting the prescribed budgets, 
We formulate our problem as a constrained optimization problem shown in Equation~\eqref{eq:opt_problem}. 
The objective is structured to minimize the difference between $\delta_d$, the desired end-to-end latency acquired from the time budgetter, and $\sum_i \delta_{i}(p_i,v_i)$, the sum of the latency across all application layer stages, $i$, as a function of their respective precision and volume $p_i, v_i$. For our MAV application, as shown previously in Table~\ref{fig:operator_table}, we have 3 application layer stages, perception ($i=0$), perception to planning ($i=1$), and planning ($i=2$).

The precision and volume chosen for each stage are subject to a series of constraints. The perception volume is limited by the perception to planning volume, which is itself limited by $v_{\text{sensor}}$ and $v_{\text{map}}$, the max volume ingested by the sensors and map, respectively. The perception precision is limited by $g_{\text{avg}}$ and $g_{\text{min}}$, the average and minimum gap size within the observed volume of space, respectively, and $d_{\text{obs}}$, the distance between the nearest obstacle and the MAV. Our framework also requires the precision for the perception to planning and planning stages to be equivalent.
%The perception stage also defines the max precision and volume we can use at any subsequent stage, and due to the constraints in our planning framework, the precision for the perception to planning and planning stages must be equivalent. Due to the constraints in our planning framework, the precision for the perception to planning and planning stages must be equivalent.
Due to the OctoMap framework's constraints, the precision values used must also be a power of two multiple of the minimum voxel size representable by the map, $vox_{\text{min}}$. The final constraint shows this for an OctoMap of depth $d$, with non-negative integer $n$.% and a non-negative integer $n$ used to select the voxel size to interpret the map at stage $i$. %Further reasoning behind these equations are omitted due to space limitations.
\begin{align} \label{eq:opt_problem}
    & \min_{p,v} \left(\delta_d - \sum_i \delta_i(p_i,v_i)\right)^2 \\
    & g_{\text{min}} \leq p_0 \leq \min(p_1, g_{\text{avg}}, d_{\text{obs}}) \nonumber \\
    & p_1 = p_2 \nonumber \\
    & v_0 \leq v_1 \leq \min(v_{\text{sensor}}, v_{\textit{map}}) \nonumber\\
    & p_i \in \{ vox_{\min} 2^n : 0 \leq n \leq d-1 \} \nonumber
\end{align}

%Solving \eqref{eq:opt_obj} finds operator settings that both meet the required deadline while making the most of the available latency budget. The set of constraints help enforce relationships between the stages and how the latency budget is allocated among them. 
%However, an expression for the system performance model for stage $i$ -- $\delta_i(\textbf{x})$ -- is needed.

%\todo{talk about how models are collected}Each one of these models are collected through having the drone to fly through various environment.

%\textbf{models}

%\todo{spend a pargraph on each model}

%\textbf{solver}
%We formulate this problem as a optimization problem. 
To find the latency of each stage, $\delta_i(p_i, v_i)$, we profiled a representative set of precision-volume combinations. 
%\red{Figure blah shows the collected data for and example stage, i.e., planner. Other stages exhibit similar behavior}.
We then fit a polynomial model to this data which had <8\% average MSE over a mission. Our model is shown in Equation~\ref{eq:model}, with coefficient vector $\textbf{q}_i \in \mathbb{R}^4$ (where $\hat{p}_i = 1 / p_i$. This change of variables is performed to improve the numerical conditioning of the optimization problem).
%simplicity, with three resolution coefficients and a single volume coefficient sufficient for a. 
%The mean squared error (MSE) of each stage's performance model is shown in \red{Figure~\ref{TODO}}. 
\begin{align}
    \delta_i(p_i,v_i) = (q_{i,0} \hat{p}_i^3 + q_{i,1} \hat{p}_i^2 + q_{i,2} \hat{p}_i) (q_{i,3} v_i) \label{eq:model}
\end{align}

\begin{comment}
For each stage, a mapping from operator settings (ie. resolution and volume) to latency is required. In order to determine this mapping, for each stage, we profile \footnote{ Profiling and model generation methodology details are presented in section blah.} the latency performance for various combinations of resolution and volume, fitting each $\delta_i(\textbf{x})$ to the following polynomial model, with coefficient vector $\textbf{q}_i \in \mathbb{R}^4$:
\begin{align}
    \delta_i(\textbf{x}) = (q_{i,0} \hat r_i^3 + q_{i,1} \hat r_i^2 + q_{i,2} \hat r_i) (q_{i,3} v_i) \label{eq:model}
\end{align}

\end{comment}

%We note that our model as defined in Equation~\eqref{eq:model} assumes that the latency of each stage is dependent only on the operator settings for the respective stage. While a conservative assumption, relaxing this assumption would only marginally improve the model while greatly increasing the model complexity as many of the interactions between the individual stage's operator settings are already captured by the constraints.


%\subsection{overhead of the design}













%\todo{spend a paragraph on each one of the priority functions and implementations}


%\todo{talk about why the objective function is setup the way it is} 
%Equation blah shows the objective function and the constraints. 
%The objective function is presented in equation blah, where delta denotes blah ... \red{go over the notation} 
%Each one of the delta denote the performance models illustrating the relationship between, space precision, volume and latency.

%Equations blah through blah list our equality and inequality constraints. 




==> tex/todo.tex <==
\begin{comment}
\todo{
The high level goal is to get a complete draft by Saturday 8/1. This includes all draft figures and story and data.
\begin{enumerate}
    \item discuss the algorith with Brian
    \item add raytracing
    \item add an appendix
    \item add the kernels in the table
    \item Intro: radhika writing a small section about the overall cyber-physical interactions. Will do the rest once everything is done.
    \item Background: will do week of deadline. Jon to respin figures.
    \item Motivation/Spatial Aware: VJ to read through for story / edits. Behzad to re-run the data. Jon to respin figures.
    \item Roborun: Behzad to write. Brian/VJ to help with story / edits. Jon to finish solver development. Jon to respin figures.
    \item Infrastructure: Radhika to write. Jon to respin figures.
    \item Results: Behzad to write. Behzad/Radhika collecting new data. Jon to respin figures.
    \item Related Work: Jon to write.
    \item Conclusion: will do week of deadline
  
  
  
  \item replace resolution with precision
 spatial-obliviuos being 78\%
  \item make sure to bring up the end-to-end ness
  \item change Zone to zone
  \item double check the figures and make sure they are all big enough
\end{enumerate}
}

places to cut down: table2 combine a bunch of rows.

\end{comment}
